Overlapping subspaces and singular systems with application to Isogeometric Analysis

We propose a framework for solving partial differential equations (PDEs) motivated by isogeometric analysis (IGA) and local tensor-product splines. Instead of using a global basis for the solution space we use as generators the disjoint union of subspace bases. This leads to a potentially singular linear system, which is handled by a Krylov linear solver. The framework may offer computational advantages in dealing with spaces like Hierarchical B-splines, T-splines, and LR-splines.

==> abstract-setting.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex

\section{Abstract setting}

We assume, for the sake of simplicity,  that \(V\) is a finite dimensional vector space
with scalar product $(\cdot,\cdot)_V$ and norm \(\n{\cdot }_V\).
%Appendix~\ref{App-1} \change{contains notes about the extension to infinite dimensional case.}{is devoted to the extension of some properties the infinite dimensional Hilbert setting.}
Recalling \eqref{eq:space}, we have spaces $V_i$, for $i=1, \ldots,
n$, such that 
\begin{displaymath}
V=\sum_{i=1}^n V_i;
\end{displaymath}
we  further  introduce the extended space 
\begin{equation}[product-space]
    \wV:=\prod_{i=1}^n V_i,
\end{equation}
endowed with the norm
\[
\n{\wv}_\wV:=\left(\sum_{i=1}^n	\n{v_i}_V^2\right)^{1/2}	,
\quad \forall 	\wv=(v_1,\dots,v_n) \in \wV.
\]

We  reformulate the abstract problem \eqref{eq:system-V} on
\(\wV\), which will lead to a linear system for the representation of
the solution with respect to  $\wPhi$ defined in
\eqref{eq:generating-system}, the basis of $ \wV $,  instead of  $\Phi$, the basis of $ V $.     {For this purpose,  each $\wv \in \wV$ is associated to
  a $v \in V$ via the following surjective operator  \(S:\wV\to V\) 
\begin{equation}[S-definition]
	S\wv=S(v_1,\dots,v_n)=\sum_{i=1}^n v_i\in V
      \end{equation}   
Its  adjoint  \(S^*:V^*\rightarrow \wV^*=\prod_i V_i^*\) is then injective and associates to \(f\) the tuple of the restrictions of \(f\) to the \(V_i\):
\[S^* f=(f|_{V_1},\dots,f|_{V_n}).\]
The \emph{extended problem} is the pull-back of {problem} 
\eqref{eq:system-V} on \(\wV\), and reads  
\begin{equation}[system-wV]
\wA \wu=\wf,
\end{equation}
where \(\wf:=S^*f\) and \(\wA:\wV\rightarrow \wV^*\) is defined by 
\begin{equation}[wA]
\wA:= S^* A S
\end{equation} 
that is 
\begin{equation}[wA-bis]
\wA (u_1,\dots,u_n)=(w|_{V_1},\dots,w|_{V_n}), \text{ with } w=\sum_{i=1}^n A u_i.
\end{equation} 


The \emph{extended problem} \change{}{, which} is equivalent to problem  \eqref{eq:system-V}  as stated in the next result.

  \begin{thm}\label{thm:system-equivalent}
    If $A:V\rightarrow V^*$ is an isomorphism, then
    \begin{equation}[ker-wA]
      \ker \wA = \ker S,
    \end{equation}
    and  
    \begin{equation}[wA-and-A-equivalence]
      Au=f \text{  if and only if } u=S \{\wu\in \wV:\wA\wu=\wf\}.
    \end{equation}
  \end{thm}
  
\begin{proof}
	Recalling that   \(S\) is surjective and  \(S^*\) is
        injective,  \eqref{eq:ker-wA} follows. Thanks to \(S^*\) being
        injective  and \(A\) an isomorphism, we also have
	\[ \wA\wu = \wf \iff S^* (AS\wu ) = S^* f \iff A S\wu=f \iff u = S\wu,\]
       which is \eqref{eq:wA-and-A-equivalence}.
\end{proof}



\section{Krylov methods}


In this section we revise and adapt to our framework the theory of
preconditioned Krylov methods,
with emphasis on  the Conjugate Gradient (CG) method,
following \cite{gunnel2014note}.
In particular, we  relate Krylov methods for the extended  problem
\eqref{eq:system-wV} to  Krylov method for the original
problem\eqref{eq:system-V}.

Assume that  a left preconditioner   \(\wB:\wV^*\to\wV\) for the extended problem
\eqref{eq:system-wV} is given. We associate to it a left preconditioner  \(B:V^*\rightarrow V\) for the
original problem \eqref{eq:system-V} as follows:
\begin{equation}
  \label{eq:defn-B-from-wB}
  B= S\wB S^*;
\end{equation}
then,  the following  commuting diagram holds
\begin{equation}[operators-cd]
    \begin{tikzcd}[sep=2cm,every label/.append style={font=\normalsize}]
        \wV \arrow[r, "\wA"] \arrow[d, "S"] & \wV^* \arrow[r, "\wB"] & \wV \arrow[d, "S"]
        \\ V\arrow[r, "A"] & V^* \arrow[r, "B"] \arrow[u, "S^*"] & V
    \end{tikzcd}
  \end{equation}
  The original and extended preconditioned operators are  $T:=BA $  and $ \wT:=\wB\wA
  $, respectively,  such that
  \begin{equation}[TS=SwT] TS=S\wT,
\end{equation}
as represented in the following commuting diagram:
\begin{equation}[operators-cd-T]
    \begin{tikzcd}[sep=2cm,every label/.append style={font=\normalsize}]
        \wV \arrow[r, "\wT"] \arrow[d, "S"] &\wV \arrow[d, "S"]
        \\ V\arrow[r, "T"]& V
    \end{tikzcd}
  \end{equation}
Finally, the  preconditioned extended
problem reads
\begin{equation}
  \label{eq:prec-ext-prbl}
  \wT \wu = \wB \wf. 
\end{equation}

Being $\wT:\wV\to \wV$  an
endomorphism on $\wV$ (though possibly singular) we can employ Krylov
methods for solving \eqref{eq:prec-ext-prbl}. Denoting $\wy = \wB \wf$,   Krylov methods provide 
at each step \(s\) an approximate solution \(\wu_s\) in the Krylov
subspace
\begin{equation}
  \label{eq:Krylov-space}
  	K_s(\wT,\wy):=\SPAN \{ \wy,\wT\wy,\dots,\wT^{s-1}\wy\},
\end{equation}
such that a suitable optimality condition is satisfied.

The convergence of Krylov methods in the singular case is not
guaranteed  in general:  it may happen  that the solution
$\wx$ of $\wT\wx = \wy $ does not belong to any Krylov space
$	K_s(\wT,\wy)$. Fortunately, this does not happen in our case under
reasonable conditions, as stated in the  following proposition. 
\begin{prop}\label{prop:krylov-convergence}
  Under the assumption that \(T\) is an isomorphisms, for all \(f
  \in V\)  the system \eqref{eq:prec-ext-prbl} admits a Krylov solution.
\end{prop}
\begin{proof}
The kernel of a composition always contains the kernel of the first map
and so by definition $$\ker \wT=\ker(\wB S^* A S )\supseteq \ker S.$$
Similarly, since \(T\) is an isomorphism and using \eqref{eq:TS=SwT}
we have 
\[
  \ker S= \ker T S= \ker  S\wT \supseteq \ker\wT.
\]
Therefore
\begin{equation}
  \label{eq:kerTbar}
  \ker \wT=\ker S.
\end{equation}
From \eqref{eq:kerTbar}, then \eqref{eq:TS=SwT}, using that
\(T\) is  an isomorphism, and finally \eqref{eq:kerTbar}  again  we have
\[
  \ker \wT^2=\ker S\wT = \ker TS=\ker S=\ker \wT,
\]
i.e., \(\ker\wT^2=\ker \wT\).
This guarantees that \cite[Theorem 2]{krylov-idea}
 $\wT \wx = \wz$ admits a Krylov solution for any \(\wz \in \range{(\wT)}\).
\end{proof}

The assumption of Theorem \ref{prop:krylov-convergence} is natural in
our framework.
In particular, $A$ is taken non-singular
by assumption,
$\wB$ is often coercive by construction
\begin{displaymath}
  \forall \wg \in \wV^*, \quad \wg \neq 0 \Rightarrow \langle \wB \wg , \wg
  \rangle > 0;
\end{displaymath}
then  $B$ is also coercive (since $ \langle B g , g
  \rangle  = \langle \wB S^* g , S^* g   \rangle  $, and $S^* $ injective) and 
  thus \(B\) is an isomorphism, which makes $T$ an
  isomorphism as well.

% This has the well known consequence that if \(\wy\) is in a
% left-invariant subspace \(\wY\), i.e. \(\wT \wY\subseteq \wY\), then
% the approximate solutions \(\wx_s\) are in \(\wY\) and, moreover, if
% \(\wT|_\wY\) is an isomorphism then the methods converge in at most
% \(\dim \wY\) iterations.

  Theorem~\ref{prop:krylov-convergence} 
assumes exact arithmetic and the exact calculation of the matrix and
right hand side of the preconditioned extended problem
\eqref{eq:prec-ext-prbl}. However,  numerical errors typically occur
and, when $\wT$ is singular, they may lead to the unsolvability of the
perturbed system. Assume, for example, that the
left-hand side of  $\wT$  is exactly computed (up to machine
precision) and the right-hand-side is affected by a quadrature
error $ \we$, that is the system reads $\wA \wu = \wf+ \we$. 
Let's further decompose $\we$  as $     \we=
  \we_{\range}+\we_{\mathscr{K}} $, with   $\we_{\range}$   in  the
  range of \(S^*\). The effect of   $\we_{\range}$  can be analyzed by means of standard methods such as the
Strang lemma, while $\we_{\mathscr{K}}$, which  is  outside the range
of \(S^*\) and then of $\wA$,
prevents  the existence of the solution of the perturbed problem. In this situation,
it is required that the stopping criterion of the Krylov iteration is  set with a
threshold on the residual norm that cannot be smaller than the norm of  $\we_{\mathscr{K}}$.




\subsection{CG and MINRES}
\change{If $A$ and $\wB$ are self-adjoint and coercive 
\begin{align}
  \label{eq:sym-pos-A} \langle A v , w  \rangle=\langle A w , v  \rangle,&\qquad \langle A v , v  \rangle >0,\, &&\forall v,w\in V,
  \\\label{eq:sym-pos-wB}\langle \wB \wv , \ww  \rangle=\langle \wB \ww , \wv  \rangle,&\qquad  \langle \wB \wv , \wv  \rangle >0,\, &&\forall \wv,\ww\in \wV^*.
\end{align}
then also $\wA$ is self-adjoint and $B$ is both self-adjoint and coercive 
\begin{align}
  \label{eq:sym-wA} \langle \wA \wv , \ww  \rangle=\langle \wA \ww , \wv  \rangle,& &&\forall \wv,\ww\in \wV,
  \\\label{eq:sym-B}\langle B v , w  \rangle=\langle B w , v  \rangle,&\qquad  \langle B v , v  \rangle >0,\, &&\forall v,w\in V^*.
\end{align}
}{
Under the conditions of symmetry and coercivity %\marginpar{\color{blue} self-adjoint?} ...
%\begin{align}
%  \label{eq:sym-pos-A} \langle A v , w  \rangle=\langle A w , v  \rangle,&\qquad \langle A v , v  \rangle >0,\, &&\forall v,w\in V,
%  \\\label{eq:sym-pos-wB}\langle \wB \wv , \ww  \rangle=\langle \wB \ww , \wv  \rangle,&\qquad  \langle \wB \wv , \wv  \rangle >0,\, &&\forall \wv,\ww\in \wV^*.
%\end{align}
it follows that $\langle \wA \cdot , \cdot  \rangle $ is also %\change{self-adjoint}{symmetric}
, while $\langle B \cdot, \cdot \rangle $ is also %\change{self-adjoint}{symmetric}
and %\change{coercive}{positive definite}.
} We can \change{indeed}{} apply CG, for which the convergence histories of the
original and extended problem coincide.
\begin{thm}\label{thm:krylov-iteration-CG} Under the assumptions above,
  let $u_s$ and $\wu_s$ be the  iterates at step \(s\)  of the
  (preconditioned) CG method applied 
  to the original problem \eqref{eq:system-V} and the extended problem
  \eqref{eq:system-wV}, respectively. Then for all $s$,
  \begin{equation}
    \label{eq:CG-equiv}
    S\wu_s= u_s
  \end{equation}
  \begin{equation}
    \label{eq:CG-equiv-norm}
    \n{\we_s}_{\wA}=\n{e_s}_A, 
  \end{equation}
where \(\we_s\in \wV\)   is  the
error at step \(s\) of the CG method applied to the extended problem,  i.e.,
the difference between a chosen solution \(\wu\) and \(\wu_s\),
while \(e_s\in V\) is  the corresponding error obtained by the CG
method applied to the original problem, and  $\n{\cdot}_{A} =
\langle A \cdot , \cdot  \rangle$ and  $\n{\cdot}_{\wA} =
\langle \wA \cdot , \cdot  \rangle$ denote the norms or seminorms
associated to $A$ and $\wA$,  respectively.
\end{thm}

\begin{proof}\color{blue}


 For any positive integer $s$, we have by definition of $T$ and $\wT$
 that
 \begin{displaymath}
    T^sS=   S \wT^s, 
  \end{displaymath}
 and then

 \begin{displaymath}
    T^sBf =   S \wT^s\wB \wf, 
  \end{displaymath}
yielding the correspondence of  the Krylov spaces generated in \(V\) 
and \(\wV\):
\begin{equation}
  \label{eq:Krylov-relation}
  K_s(T,Bf)  = S K_s(\wT,\wB \wf).
\end{equation}
By construction any CG solution of \eqref{eq:system-V},
respectively,\eqref{eq:system-wV} fulfill the following optimality condition 
\[  u_s = \argmin_{v \in K_s(T,Bf) } \n{u - v }_{A},\quad\text{and}\quad \wu_s \in \argmin_{\wv \in K_s(\wT,\wB \wf)} \n{\wu - \wv }_{\wA}
\]
By \eqref{eq:Krylov-relation} and
\[
\n{\wv}_{\wA}^2=\langle \wA \wv , \wv  \rangle = \langle A S \wv ,
S \wv  \rangle  = \n{S \wv}_{A}^2.
\]
we have $S\wu_s=u_s$, i.e., \eqref{eq:CG-equiv} and \eqref{eq:CG-equiv-norm}.
%\eqref{eq:wA-and-A-equivalence} and ,
%\[= \argmin_{
%    \scalebox{0.8}{$\begin{aligned}
%      v &= S \wv \text{ such that } \\ \wv &\in K_s(\wT,\wB \wf)
%    \end{aligned}$}} \n{u - v }_{A}\]
%for any solution  $\wu \in \wV$ of \eqref{eq:system-wV}.  Then
% follows immediately 
%from 

\color{black}
\end{proof}

In a similar way, but without the need of \change{coerciviness}{the positive definiteness} of
$\langle A \cdot , \cdot  \rangle $, i.e., assuming only that \(A\) is
a \change{ self-adjoint}{} isomorphism satisfying
\begin{equation}
  \label{eq:sym-A} \langle A v , w  \rangle=\langle A w , v  \rangle,\qquad \forall v,w\in V,
\end{equation}
we can still apply MINRES and have the following equivalence.

\begin{thm}\label{thm:krylov-iteration-MINRES} Under the assumptions \eqref{eq:sym-A},
  \eqref{eq:sym-pos-wB},  let $u_s$ and $\wu_s$ be the  iterates at step \(s\)  of the
  (preconditioned) MINRES method applied 
  to the original problem \eqref{eq:system-V} and the extended problem
  \eqref{eq:system-wV}, respectively. Then for all $s$,
  \begin{equation}
    \label{eq:MINRES-equiv}
    S\wu_s= u_s
  \end{equation}
  and 
  \begin{equation}
    \label{eq:MINRES-equiv-norm}
   \n{\wr_s}_{\wB}= \n{r_s}_B,
  \end{equation}
where \(\wr_s\in \wV^*\) is the residual at step \(s\) of the MINRES
method applied to the extended problem, \(r_s\in V^*\)  is the residual of the MINRES method applied to the original problem  and  $\n{\cdot}_{B} =
\langle B \cdot , \cdot  \rangle$ and  $\n{\cdot}_{\wB} =
\langle \wB \cdot , \cdot  \rangle$ denote the norms 
associated to $B$ and $\wB$,  respectively.
\end{thm}

\color{blue}
\begin{proof}
As shown in \eqref{eq:Krylov-relation} the Krylov subspaces correspond by \(S\).
Similarly to the CG, any MINRES solution of \eqref{eq:system-V},
respectively,\eqref{eq:system-wV} fulfill the following optimality conditions
\[
    u_s = \argmin_{v \in K_s(T,Bf) } \n{A v - f }_{B},\quad\text{and}\quad
\wu_s \in \argmin_{\wv \in K_s(\wT,\wB \wf) } \n{\wA \wv - \wf }_{\wB}
% = \argmin_{
%      \scalebox{0.8}{$\begin{aligned}
%        v &= S \wv \text{ such that } \\ \wv &\in K_s(\wT,\wB \wf)
%      \end{aligned}$}
%  } \n{ Av - f }_{B},
\]
%and
%\[\begin{aligned}
%    \wu_s =& \argmin_{\wv \in K_s(\wT,\wB \wf) } \n{\wA \wv - \wf }_{\wB}
%      = \argmin_{\wv \in K_s(\wT,\wB \wf) } \n{ S^* (A S \wv - f) }_{\wB}
%      \\=& \argmin_{\wv \in K_s(\wT,\wB \wf) } \n{ A S \wv - f }_{B}.
%\end{aligned}\]
By \eqref{eq:Krylov-relation}, \(\n{S^*v }_{\wB}= \n{v}_{B}\)
and
\[
\wA\wv-\wf=S^*(AS\wv -f)
\]
we have $S\wu_s=u_s$, i.e., this proves \eqref{eq:MINRES-equiv} and \eqref{eq:MINRES-equiv-norm}.
\end{proof}
\color{black}

\subsection{GMRES}


The standard GMRES method minimizes at
each step the euclidean norm of the residual.
It follows that the iterate are basis dependent and differ between the
original and the extended problem.
% \footnote{Results
% similar to Theorem~\ref{thm:krylov-iteration-CG} and \ref{thm:krylov-iteration-MINRES}
% can be obtained with GMRES if \(\wB\) satisfies \eqref{eq:sym-pos-wB}
% and defines a norm.
% This is not a natural assumption in the context of a non-symmetric
% problem. Another possibility is to have an implementation in
% which the scalar product for the residual is explicit, but this is not
% common in linear algebra libraries. *** nota da discutere, io sarei
% piu per togliere ***} 
At the same time, the behavior of GMRES mainly depends on the spectrum of the
preconditioned problem, which is the same for the two problems,
original and extended, up to the possible kernel of the latter.
% This
% is stated in the following proposition for the left-preconditioned
% case, though a similar results hold for the right preconditioned.

\begin{thm}\label{thm:preconditioner-spectrum}
Under the assumption that  \(T\) is an isomorphism, the spectrum
$\spectrum(\wT) $  of \(\wT\), and the spectrum $\spectrum(T) $   of \(T\) are related by
	\[\spectrum(\wT)\setminus\{0\}=\spectrum(T).\]
\end{thm}

\begin{proof}
For \(\lambda\in\spectrum(\wT)\setminus\{0\}\) there exists
\(\wv_\lambda\not\in \ker S\) such that  \(\wT\wv_\lambda=\lambda\wv_\lambda\). 
	From \eqref{eq:TS=SwT} \[T S\wv_\lambda= S\wT\wv_\lambda =\lambda S \wv_\lambda\]
	and we see that \(S\wv_\lambda\) is an eigenvector for \(T\) and \(\lambda\in\spectrum(T)\). Thus \(\spectrum(\wT)\setminus\{0\} \subseteq \spectrum(T)\).


        Similarly if \(\lambda\in\spectrum(T)\) there exists
        \(w_\lambda\ne 0\) such that  \(\lambda w_\lambda= T
        w_\lambda\). Let
          \begin{equation}
            \label{eq:wwlambda1}
            \ww_\lambda = \lambda^{-1} \wB S^* A
          w_\lambda,
          \end{equation}
          then we have
          \begin{equation}
              \label{eq:wwlambda2}
            S \ww_\lambda = \lambda^{-1} S \wB S^* A w_\lambda =
            \lambda^{-1} T  w_\lambda =  w_\lambda
          \end{equation}
          and therefore, using \eqref{eq:wwlambda2} and then \eqref{eq:wwlambda1}
          \begin{displaymath}
            \wT \ww_\lambda =   \wB S^* A S \ww_\lambda = \wB S^* A
            w_\lambda= \lambda \ww_\lambda 
          \end{displaymath}
therefore  \(\lambda \in\spectrum(\wT)\).
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "easy_adaptivity_and_solver_v8"
%%% End:


==> conclusions.tex <==
\section{Conclusions}

One interesting further work is to combine RB-splines as proposed here
with  the case  when  tensor-product patches overlap in the physical domain that is, subspaces of 
isogeometric functions (isoparametrically mapped tensor-product  splines) with
different parametrization for different patches are merged. This is
the typical setting of multipatch geometries and can be coupled with
iterative solvers as in \cite{bercovier2015overlapping} and  presents different difficulties: typically we do not
encounter linear dependencies in the set of generating functions, when
the overlapping meshes are not aligned, but accurate integration or
projection between overlapping subspaces are still an open challange.



==> efficient.tex <==
\subsubsection{A priori estimates}

The proposed approach does not necessarily work well and for this it is worth to study for a given $V$ the depence of $K$ and $\C$ on the collection of the $V_i$.

% Theorem~\ref{thm: classical-result} have a nive geometric interpretation

\begin{lem} Let \(\widetilde{V}_i\), \(i=1,\dots,n\) be such that
\[
\widetilde{V}_i\supseteq V_i,\qquad V=\sum_i\widetilde{V}_i=\sum_i V_i,
\]
then 
\[\widetilde K \le K, \qquad \widetilde{\C}\ge \C.\]
\end{lem}

\begin{proof}
Replacing \(V_i\) with a supset \(\widetilde V_i\) corresponds to a bigger set of inverses in \eqref{eq:stable-dec} and to a bigger space in \eqref{eq:s-cauchy-schwarz}. This emplies that \(K\) being the infimum is smaller or equal to and that the norm of \(\C\) increases as it is a monotone function of the positive entries.
\end{proof}

If $V$ has a Sobolev norm the scalar product of spaces with non-overlapping support is zero. Let $\support V_i$ be
\[
\support V_i:=\bigcup_{f\in V_i} \support f.
\]

\begin{lem} The Cauchy-Schwarz positive symmetric matrix is bounded from above by
\[
\C\le U, \qquad U_{i,j}=\begin{cases} 1 & \mu(\support V_i\cap \support V_j) >0
\\ 0&\text{otherwise}.\end{cases}
\]
And $\n{\C}_{\R^n\to\R^n}$ is bounded by the maximum number of overlapping patches:
\[
\n{\C}_{\R^n\to\R^n}\le \n{U}_{\R^n\to\R^n}\le \max_i\{\sum_j M_{i,j}\}.
\]
\end{lem}

\marginpar{It is relatively easy to give a error estimate for the greedy-SSC based on the minimal angle. Should we do it? {\color{blue} Mi rispondo da solo, no} {\color{red}forse sì}}

\color{blue}
For elliptic self adjoints problems, the greedy SSC acts as
an iterative solver whose convergence depends only on
the set of the $V_i$ and the number of steps.

Indeed let \( \C_{\min} \) be the minimum cosine between a vector \(v\in V\) and the \(V_i\):
\[
    \C_{\min}:= \inf_{v\ne 0 \in V}\max_i \sup_{w_i\ne 0\in V_i} \frac{a(v,w_i)}{\n{w_i}_a \n{v}_a}
\]
The best possible bound on 

\begin{lem}\label{thm:S-inverse-norm}
    For all \(v\in V\) there is \(\wv\in S^{-1}v \) satisfying 
\[
    \n{\wv}_\wA\le \frac\rho{1-\rho}\n{v}_A.
\]
and \(\rho=\sqrt{1-\C_{\min}^2}\).

\end{lem}

\begin{proof}
For all \(v\in V\) 
\[
    \n{v}_a^2=\n{T_i v}_a^2 + \n{v-T_i v}_a^2
\]
so that by choosing \(i\) that maximize \(\n{T_i v}_a^2\) we have
\[
    \n{v-T_i v}_a^2\le (1-\C_{\min}^2)\n{v}_a^2 \quad\thus\quad \n{v-T_i v}_a\le\rho\n{v}_a.
\]
Then starting from \(v\in V\) we build \(\wv\) as the limit of
\(\wBs^{[k]} S^* A v\) where \(\wBs^{[k]}\) corresponds to the \(v\) dependent 
sequence of steps \(i_1,\dots,i_k\) with the property that at each step
the norm of \( \n{T_{i_j}\wBs^{[j-1]} S^* A v S v}_a^2 \) is maximized.

It follows that \(\n{v-\wBs^{[k]} S^* A v}_a\le \rho^k \) and 
\[
\n{\wv}_a= \n{\sum_{j} \wT_{i_j} (\Id-\wBs^{[j-1]} S^* A) v }_a\le \sum_{j=1}^{\infty} \rho^j.
\]
\end{proof}

\color{black}

==> elliptic-case.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex


\subsection{Elliptic case}

The analysis of the subspace correction methods for elliptic problems is the
most known, see for instance \cite{Xu1992,MR2104179}. 
Here we recall the usual theoretical framework, that is a special case of
Theorem~\ref{thm:PSC-spectrum} and \ref{thm:SSC-error}.

We consider in particular an elliptic equation in an Hilbert space 
\(H\supset V\) \marginpar{USIAMO DIRETTAMENTE \( V\) ED EVITIAMO LA
  BEN NOTA DISCUSSIONE SUL METODO DI GALERKIN?}: find \(u\in H\) such that
\begin{equation}[problem-hilbert]
    a(u,v)=f(v),\qquad \forall v\in H,
\end{equation}
where \(a\) is a symmetric positive definite bilinear form such that
\[a(v,v)\ge\alpha \n{v}_H^2,\] and \(f\in H^*\).
The bilinear form \(a\) is a scalar product on \(V\) that induces a 
norm that is equivalent to the norm on \(V\)
\begin{equation}
\n v_a^2:=a(v,v).
\end{equation}
Problem \eqref{eq:system-V} is obtained by introducing \(A:H\to H^*\) defined by
the equation \[ (Au)(w)=(u,w)_H,\ \forall w\in H\] and restricting it to the space \(V\).
By the Ceá Lemma the distance between the solution \(u\in H\) of the original problem and that of the restricted problem \(u_V\in V\) is bounded
\[
\n{u-u_V}_H \le \frac{\n A ^{1/2}}{\alpha^{1/2}} \inf_{w\in V}\n{u-w}_H.
\]

The analysis of the PSC method often done with respect of the \(A\)
induced norm.\marginpar{QUANTO SEGUE E`  DA LEGARE A QUANTO NELLE
  SEZIONI PRECEDENTI...}
To apply Lemma~\ref{thm:stable-decomposition} one assumes the existence of 
\emph{stable-decompositions}, i.e. for all \(v\in V\)
exists \(\wv=(v_1,\dots,v_n)\in S^{-1}v\) such that
\begin{equation}[stable-decomposition]
\sum_{i=1}^n (R_i^{-1} v_i,v_i) \le K_0\, a(v,v)=K_0 \n v_a^2,
\end{equation}
that, by Lemma~\ref{thm:stable-decomposition}, directly implies \(\min \spectrum(\Tp)\ge K_0^{-1}\).
The upper bound on \(\spectrum(\Tp)\) is achieved assuming the
\emph{strengthened Cauchy-Schwarz inequality}
\begin{equation}[strengthened-CS]
    \begin{aligned}
        a(S\wTp \wu,S\wTp \wv) &\le K_1 \Big(\sum_{i=1}^n a(T_i v_i, v_i)\Big)^{1/2} \Big(\sum_{i=1}^n a(T_i u_i, u_i)\Big)^{1/2}.
    \end{aligned}
\end{equation}
that leads to \(\n{Tv}_a^2 \le K_1 \n{Tv}_a \n{v}_a\) and \(\max \spectrum(\Tp)\le K_1\).
In practice \(K_1\) is analyzed by using Proposition~\ref{thm:psc-upper-estimate}.

Finally the norm of the error operator \(\Es=\Id-\Ts\) is bounded in terms
of \(K_0,K_1\) and the norm of the operators \(T_i\), see for instance \cite[Theorem~4.4]{Xu1992} 
\begin{equation}
    \n{E}^2\le \frac{2-\max\{ \n{T_i}_{V\to V_i},\, i=1,\dots,n\}}{K_0(1+K_1)^2}.
\end{equation}

*** sono arrivato qui ***

A questo punto si potrebbe mettere il caso ellittico, IGA e i test
numerici tutti nella stessa sezione?

*************************

\change{}{
    For reasons that will be clear later let also
    \begin{equation}
    \omega_0:=\max \{\n{T_i^{-1}},\, i=1,\dots,n \}.
    \end{equation}
        

To solve the equation we propose to choose some spaces \(V_i\) and construct the
matrix representation with respect to the basis \(\wPhi\) of \(\wV\).
Let \[
    A_i :V_i\to V_i^*,\qquad A_i v_i=A v_i|_{V_i},
    \]
be the operator corresponding to the restriction of \eqref{eq:problem-hilbert} to \(V_i\) and \(R_i:V_i^*\to V_i\) be an self-adjoint and positive definite
\[R_iv_i(v_i)=0\iff 0=v_i\in V_i.\]

Following the theory of PSC and SSC described in \cite{Xu1992} the properties of the spectrum of the preconditioned system \eqref{eq:system-V-prec} using \(B_p\) and \(B_s\) are determined how well \(R_i\) approximate the inverse of \(A_i\), the \emph{strengthned Cauchy-Schwarz} inequality and the \emph{stable-decomposition}.
These properties are here rewritten in the our framework in view of Theorem~\ref{thm:system-equivalent}, \ref{thm:preconditioner-spectrum} and \ref{thm:krylov-iteration}.

Since the \(R_i\) are self-adjoint and positive definite their distance from  \(A_i^{-1}\) is measured by the spectrum of \(R_iA_i\).
Let
\begin{equation}
\begin{aligned}
&\omega_1:=\max_{i=1}^n\{\lambda_{\max}(R_i A_i)\},
\\&\omega_0:=\max_{i=1}^n\{\lambda_{\min}(R_i A_i)^{-1} \}.
\end{aligned}
\end{equation} 
In our framework, the existence of stable decompositions can be rewritten as the existence of bounded inverses of \(S\) in the \(a\)-induced norm: for all \(v\in V\) exists \(\wv=(v_1,\dots,v_n)\in S^{-1}v\) such that
\begin{equation}%[stable-decomposition]
\sum_{i=1}^n (R_i^{-1} v_i,v_i) \le K_0\, a(v,v)=K_0 \n v_a^2
\end{equation}
The strengthened Cauchy-Schwarz inequality reads as
\begin{equation}%[strengthened-CS]
\begin{aligned}
 a(S\wT_p \wu,S\wT_p \wv) &\le K_1 \Big(\sum_{i=1}^n a(R_i A_i v_i, v_i)\Big)^{1/2} \Big(\sum_{i=1}^n a(R_i A_i u_i, u_i)\Big)^{1/2}.
 \end{aligned}
\end{equation} 

For the parallel subspace correction one gets by standard arguments that \(B_p\) is self-adjoint, positive definite and moreover
\begin{thm}[4.1 from \cite{Xu1992}]\label{thm:standard-theory-PSC}
The spectrum of the operator \(T_p:=B_pA\) associated to the PSC method satisfies
\begin{equation}[standard-theory-PSC]
\spectrum(T_p)\subseteq [K_0^{-1}, K_1],
\end{equation}
and consequently \(\cond(T_p)\le K_0K_1\).
\end{thm}

For the subsequent subspace correction the preconditioner \(B_s\) is self adjoint iff the sequence \(i_1,\dots,i_J\) is palindrome, for this it is usually set to \((1,2,\dots,n-1,n,n-1,\dots,2,1)\).
\begin{thm}[4.4 from \cite{Xu1992}]\label{thm:standard-theory-SSC}
Let \(T_i=R_i A|_{V_i}\) and  \(\omega_1=\max_{i=1}^n\{\n{T_i}\} \), then the norm of the error operator \(E:V\rightarrow V\) of the SSC method 
\[
E:=\prod_{i=1}^J(I-T_i)
\]
 satisfies
\begin{equation}[standard-theory-SSC]
\n{E}^2\le \frac{2-\omega_1}{K_0(1+K_1)^2}.
\end{equation}
\end{thm}
}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "easy_adaptivity_and_solver_v6"
%%% End:


==> iga.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex

\section{Application to IGA}

\change{
IsoGeometric Analysis is a Gaerlkin method for the solution of PDEs.
The domain \(\Omega\subset\R^n\) of the PDE is described as the union of disjoint possibly \emph{trimmed} patches.
Each patch is the image of a map \([0,1]^d\to\Omega\).
The pull-back of the PDE to \([0,1]^d\) is solved
using a spline discretization on \([0,1]^d\).
We focus only on untrimmed patches and for simplicity we will focus
mostly on the single patch case.

When tensor-product splines are employed, and this is the usual case,
the implementation is simplified and the computational time can be
greatly reduced by the combination of different techniques.

By employing specialized integration techniques such as \emph{sum-factorization}
and \emph{weighted-quadrature}, see \cite{MR3610113,bressan2019-sf},
the assemblying of the system matrix and also its \emph{matrix-free} application can be computed with a reduced cost, expecially for high polynomial degree.

Moreover if the pulled-back PDE is an \(L^2\)-projection or a
Poisson problem, e.g. when the patch-map is affine, then one can exploit the Kronecker-structure of the
operator on \([0,1]^d\) and solve the problem with a very small computational cost by mean of \emph{fast-diagonalization}(FD)\cite{???}.
FD reduces the Poisson PDE to the one-dimensional case and 
the solution of the multivariate problem can be obtained in (almost) linear cost on the space dimension.
More generally one can use the fast-diagonalization Poisson-solver
as a inexact solver for the pulled-back PDE. 
\marginpar{@Giancarlo cosa citare qui?}
}{Isogeometric analysis is mostly done with tensor product B-spline basis.
The tensor product structure, not only simplifies the implementation, but also allows for the use of \emph{sum-factorization}, \emph{weighted-quadrature} and a \emph{matrix-free} approach where the application of \(A\) is computed directly\cite{MR3610113,bressan2019-sf} saving both memory and time when weighted quadrature is employed.

By exploiting their Kronecker structure the inversion of the mass and stiffness matrices on the parametric domain, i.e. of the $L^2$ projection and the Poisson problem, can be reduced to the one-dimensional case and so it can be done at (almost) linear cost on the space dimension.
These fast inversion techniques can then be used as preconditioners in the physical domain.This is called \emph{fast-diagonalization} \cite{???}.} 

\change{The idea is to use tensor product splines for the \(V_i\),
so that by restricting the domain and changing the resolution of the \(V_i\) adaptivity is achieved
without the complexity of non-tensor-product spline spaces, such as hierarchical B-splines, T-splines or LR-splines and while exploiting existing fast algorithms.}{
The appeal of the proposed framework for IGA applications is the possibility to achieve adaptivity without the complexity of non-tensor-product spline spaces, such as hierarchical B-splines, T-splines or LR-splines and while keeping the simple and optimized techniques for tensor product B-splines on each patch.

The interest is thus in using tensor product B-spline patches for the \(V_i\).}
\change{More in detail the proposal is to overlap }{
The usual case is that }a coarse global patch \(V_0\) on \([0,1]^d\) \change{with }{is enriched by adding }other patches \(V_i\) of function supported on \(\Omega_i\) that extend to \(0\) on \([0,1]^d\) with the same number of continuous derivatives as \(V_0\).
\change{In particular }{I.e., }if the $k$-method is employed \change{the generating functions of $V_i$ have}{} $(p-1)$ \change{continuous}{} derivatives \change{on \((0,1)^d\)}{of the functions in \(V_i\) are zero on \(\partial \Omega_i \cap  (0,1)^d\).}

The discretization is then \(V=\sum_i V_i\) where the are tensor product B-spline patches.
The extended matrix has the following block form
\[
\wA=\begin{pmatrix}
	A_{1,1} & \dots & A_{1,n}\\
	\vdots & & \vdots\\
	A_{n,1} &\dots & A_{n,n}\end{pmatrix}\bigskip
\]
where \(A_{i,j}\) is the Petrov-Galerkin matrix of \(A\) for the pair \((V_i,V_j)\)
so that the optimized-assembling or matrix-free-application algorithms can be employed.
The subspace correction methods are constructed either with direct solvers \(R_i\) for the diagonal blocks \(A_{i,i}\) or by the fast-diagonalization method.

\change{}{The advantage of these optimized techniques are more and more clear as the polynomial degree is increased: the cost of matrix vector application with weighted quadrature and sum factorization (either global or using row-by-row assembling) is as low as $O(p \dim V_i)$ while the application of fast diagonalization preconditioner has a cost of order $O(p (\dim V_i)^{4/3})$.

Then the cost of a CG, MINRES o GMRES iteration is of order \[O(p \sum_i(\dim V_i)^{4/3})\le O(p (\dim \wV) (\max_i (\dim V_i)^{1/3}),\]
while the number of iterations is determined by \(K\) and \(\n{\C}_{\R^n\to\R^n}\) in Theorem~\ref{thm:classical-result} and the domain geometry that influences \(\lambda_{\min}\) and \(\lambda_{\max}\).}

At the moment a good strategy in the choice of the \(V_i\) is still in development, but the numerical tests for the Poisson problem with homogeneous Dirichlet boundary conditions show that it is possible to achieve convergence with few iterations.
A solution should take into account the contrasting effects of a larger space due to linear dependencies and the conditioning of that gets better as the patches overlap more and in a ``compatible'' way.

\color{black}

==> intro.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex

%\marginpar{Ho inserito il comando  \textbackslash change\{aggiunto\}\{rimosso\} per far risultare le modifiche. La parte rimossa è scritta a margine Se chi fa il passaggio successivo approva la modifica può sostituire il comando con il primo argomento.}


\section{Introduction}

In this paper we consider a non-standard framework for numerical methods for PDEs, motivated by isogeometric analysis based on   hierarchical splines or extensions with a local tensor structure.

At an abstract level, consider the problem: find \(u\in V\) such that 
\begin{equation}[system-V]
Au=f,
\end{equation}
where \(A:V\rightarrow V^*\) is a linear operator  and \(f\in V^*\), with $V$  a Hilbert space. When  \eqref{eq:system-V} represents a numerical scheme, $V$  is also finite dimensional. It is then straightforward to rewrite  problem \eqref{eq:system-V} in matrix form by choosing a basis \(\Phi\) of \(V\). Instead, we take a different path, further assuming that  \(V\) is given  as the sum of {closed} subspaces \(V_i \subset V\), \(i=1,\dots,n\)
\begin{equation}[space]
V=\sum_{i=1}^n V_i,
\end{equation}
and that  we have a basis \(\Phi_i\) for each space \(V_i\). We then consider the the disjoint union
\begin{equation}[generating-system]
  \wPhi=\coprod_{i=1}^n \Phi_i
\end{equation}
that in general is not a basis for $V$, since their elements can be linearly dependent and even be duplicated.  We can represent the solution $u$ as linear combination of elements of $ \wPhi$ and, using $ \wPhi$  instead of $ \Phi$, write  \eqref{eq:system-V} as a linear system, that may be singular.  Therefore such a linear system can not be solved by standard direct methods, while can be treated without difficulty \marginpar{\color{red}``without difficulty'' non \`e troppo ottimista?}
by iterative methods. In fact, iterative methods, especially Krylov ones, represent nowadays the most efficient solvers, when  a good preconditioner is available. We construct such a  preconditioner from the approximate solution of the restrictions of $A$ to each $V_i$, following  the well-known  subspace correction technique. Furthermore, by careful choosing the \(V_i\), as explained later,  we simplify the implemetation and improve performances. In conclusion, we are able to gain versatility and computational efficiency,   at the cost of losing the  comfort of the non-singular linear system.

\marginpar{\color{blue}@Giancarlo, cosa volevi citare qui?}
The framework outlined above is not standard but also not new  in literature. The 1994  paper \cite{griebel1994multilevel} by  Griebel proposed, in the context of finite elements, to abandon the basis in favor of a  generating system as \eqref{eq:generating-system} in order to simplify the construction of the preconditioner. Later, ??? have used generating systems in the context of wavelets methods, and ??? in the context of sparse grid. 

In the present  paper we adapt the ideas above to isogeometric analysis (IGA), and show how to exploit its advantages. IGA, introduced  in 2005 \cite{hughes2005,cottrell2009isogeometric}, has been aimed at narrowing the existing gap between numerical simulations and Computer Aided Design (CAD).  Specifically, IGA follows the isoparametric paradigm  and adopts B-splines (or NURBS and other splines extensions) as basis functions. In this way,   the unknown fields of the numerical simulation are represented by splines as, in CAD, splines are used to  parametrize the  geometry of interest.

In IGA and CAD, it is typical that each  patch is obtained  from a  tensor product basis. There are however  spline extensions proposed  for mesh refinement, such as  Hierarchical B-splines \cite{forsey1995surface,vuong2011hierarchical,buffa2016adaptive}, T-splines \cite{sederberg2003t,MR3519556,MR3084741,MR3341848}, LR-splines \cite{MR3019748,MR3146870,MR3370382}: these spaces typically have a  local tensor product structure, 
\marginpar{\color{red} ...in realt\`a ci possono essere spazi senza nessuna struttura prodotto-tensore, a parte quella delle singole funzioni di base...}
that is, the space on each patch is the union of tensor product  subspaces \(V_i\). In our paper,  the tensor product structure of the  \(V_i\)  is exploited for the fast solution of the related subproblems (that is, the restriction of $A$ to each $V_i$), for preconditioning.  With this approach it is straightforward to work with the  subspace bases  $\Phi_i$ and their disjoint union $ \wPhi $, which is particularly beneficial when it is not easy to identify the global  basis $\Phi$, as  with anisotropic refinement as in \cite{engleitner2017patchwork,engleitner2019lofting,MR3723028}.

The main ingredients of our approach were already known, but  their combination looks promising for the  development of  isogeometric solvers with a good balance of  computational efficiency and flexibility.   At a modest cost in mesh versatility and number of degrees of freedom, by working on a suitable  collection  $\wPhi$  of bases we retain the computational advantage of a tensor product structure and  gain generality, e.g., with the ability of anisotropic refinement, the possibility of overlapping spaces with different directional resolution like in adaptive sparse grids \cite{MR3785510}.


{\color{blue}
Section~2 describes the framework and sets the notation. Sections~3 and 4 rephrase Krylov methods and subspace correction preconditioners in the proposed framework highlighting the convergence properties and recalling the most important results for elliptic self-adjoint problems.

Section~5 focus on IGA applications and the possible techniques that can be carried over from the tensor product space to the current framework. In Section~6 we report on some numerical examples that show both the strengths and some weaknesses of the proposed approach.

}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "easy_adaptivity_and_solver_v8"
%%% End:


==> numerical-examples.tex <==
% !TEX root = easy_adaptivity_and_solver_v8.tex

\section{Numerical examples}
\marginpar{\color{red} Se introduciamo la mappa, dobbiamo decidere che notazione usare per gli spazi, dato che i precondizionatori sono costruiti con gli spazi non mappati...}

The numerical tests consists in the solution of the following variational Poisson problem:
\begin{equation*}
 \text{find} \; u \in V \subset  H^1_0(\Omega) \quad \text{s.t.} \int_{\Omega} \nabla u \cdot \nabla v \, d\Omega = \int_{\Omega} f v  \, d\Omega \quad \forall v \in V \, ,
\end{equation*}
where $\R^d \supset \Omega = F([0,1]^d) $ ($d=2,3$), $f = \hat{f} \circ F^{-1}$, $\hat{f} \colon [0,1]^d \to \R$ is a piecewise-constant function (with random constant coefficients over a uniform $4^d$ tessellation of the parametric domain $[0,1]^d$). \marginpar{Secondo me non \`e chiaro com'\`e definita $f$...}


The different cases relate to the choice of the test and trial space $V$ and/or the mapping function $F$.

\begin{remark}
For all cases the iterative linear solver was stopped when the discrete residual was $< 10^{-11}$ or the number of iterations reached the upper limit of $1000$.
\end{remark}

\begin{remark}
 The number of dofs refers to the dimension of $\wV$ (the dimension of $V$ is smaller).
 \marginpar{estendere la discussione?}
\end{remark}


%\subsection{Local refinement}\label{ex:local-refinement}

%\subsection{Anisotropic refinement}\label{ex:anisotropic-refinement}

\subsection{Case ???: 2D, polar mapping, anisotropic refinement} \label{sec:test_2D_1}
For this case $d=2$ and $\Omega$ is the image of the parametric domain $$\widehat\Omega := [1,2] \times [\frac{\pi}{4},\frac{3 \pi}{4}] $$ under the polar mapping $$F(\rho,\theta) = \bigl( \rho \cos(\theta), \rho \sin(\theta) \bigr)^T.$$
The test and trial space $V$ is defined as $V = V_0 + \sum_{k=1}^n \bigl( V_k^{x} + V_k^{y} \bigr)$, where:
\begin{itemize}
  \item $V_0$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat\Omega$ with uniform knots vectors of size $\frac{1}{2^{L+2}} (1, \frac{\pi}{2})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The correspondent physical domain of this space is depicted in Fig.\ref{fig:2d_V0};
  \item $V_k^{x}$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat{\Omega}_k^x = [ 1,\frac{3}{2} ] \times [ \frac{\pi}{4},\frac{\pi}{4} \bigl( 1 + \frac{1}{2^{k-1}} \bigr) ]$, with uniform knots vectors of size $\frac{1}{2^{L+2}} (1, \frac{\pi}{2^{k+1}})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The physical domains corresponding to the spaces $V_1^{x}$ and $V_2^{x}$  (with $L=0$) are depicted in Fig.\ref{fig:2d_V1x} and Fig.\ref{fig:2d_V2x}, respectively;
  \item $V_k^{y}$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat{\Omega}_k^y = [ 1,1 + \frac{1}{2^k} ] \times [ \frac{\pi}{4},\frac{5 \pi}{8} ] $, with uniform knots vectors of size $\frac{1}{2^{L+2}} (\frac{1}{2^k}, \frac{\pi}{2})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The physical domains corresponding to the spaces $V_1^{y}$ and $V_2^{y}$ (with $L=0$) are depicted in Fig.\ref{fig:2d_V1y} and Fig.\ref{fig:2d_V2y}, respectively.
\end{itemize}
Note that with this choice, the meshes related to $V_k^{x}$ and $V_k^{y}$ have the same number of elements, independently from $k$.

We tested the proposed method with $n = 2$ (corresponding to 5 overlapping domains) with different values of the mesh parameter $L$ for degrees $p=2$ (Table~\ref{table:aniso_2D_deg2_n2}) and $p=3$ (Table~\ref{table:aniso_2D_deg3_n2}), where can be observed that the use of the symmetric Gauss-Seidel preconditioner in the Conjugate Gradient solver gives us a substantial advantage (in term of number of required iterations) with respect to the strategy with no preconditioner. 
We can also observe that, in both cases $p=2$ and $p=3$ the number iterations needed for the convergence of the preconditioned approach increase for the coarser meshes (i.e. low values of $L$) and then remain almost constant for the finer meshes, as expected. Another observation is the fact that the number of iterations increases with $p$, meaning that the proposed method is not $p$-stable.

\begin{figure}
  \centering
  \includegraphics[width=.4\linewidth]{figures/plot_2d_00.png}
  \caption{2D case: the physical domain $F(\widehat{\Omega}_0)$ associated to the space $V_0$ for $L=0$.}
  \label{fig:2d_V0}
\end{figure}

\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_2d_x_liv1.png}
  \caption{$F(\widehat{\Omega}_{1,x})$}
  \label{fig:2d_V1x}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_2d_x_liv2.png}
  \caption{$F(\widehat{\Omega}_{2,x})$}
  \label{fig:2d_V2x}
\end{subfigure}
\vfill
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_2d_y_liv1.png}
  \caption{$F(\widehat{\Omega}_{1,y})$}
  \label{fig:2d_V1y}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_2d_y_liv2.png}
  \caption{$F(\widehat{\Omega}_{2,y})$}
  \label{fig:2d_V2y}
\end{subfigure}%
\caption{2D case: the different physical domains associated to the spaces $V_{1}^x$ (\ref{fig:2d_V1x}), $V_{2}^x$ (\ref{fig:2d_V2x}), $V_{1}^y$ (\ref{fig:2d_V1y}) and $V_{2}^y$ (\ref{fig:2d_V2y}) for $L=0$.}
\label{fig:2d_phys_domains}
\end{figure}





\pgfplotstableset{create on use/NewColL2D/.style={create col/set list={0,1,2,3,4,5,6,7},},columns/NewColL2D/.style={string type},}


%--------------------------------------------------------------------------------------------------------------
% 2D, degree=2
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=2_deg_max=2_nlevels_min=2_nlevels_max=2_polar_map_gauss_seidel.dat}{\dataAnisoTwoDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 11}
%]{13}{\dataAnisoTwoDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 12}
%]{14}{\dataAnisoTwoDdegTwo}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={NewColL2D,7,9,10,11,12},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/NewColL2D/.style={
      column name=$L$,
      int detect},
%    columns/1/.style={
%      column name=$h^{-1}$,
%      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
  ]
  {\dataAnisoTwoDdegTwo}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}
  \caption{2D case: dependency of the number of iterations of the Conjugate Gradient (CG) method and with symmetric block Gauss-Seidel preconditioner (PCG-GS) 
  %and with block-Jacobi preconditioner (PCG-J)) 
  w.r.t. the mesh parameter $L$, for the case with degree $p = 2$ and $n=2$ (i.e. $5$ overlapping domains).} \label{table:aniso_2D_deg2_n2}
\end{table}


%--------------------------------------------------------------------------------------------------------------
% 2D, degree=3
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_polar_map_gauss_seidel.dat}{\dataAnisoTwoDdegThree}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 11}
%]{13}{\dataAnisoTwoDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 12}
%]{14}{\dataAnisoTwoDdegTwo}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={NewColL2D,7,9,10,11,12},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/NewColL2D/.style={
      column name=$L$,
      int detect},
%    columns/1/.style={
%      column name=$h^{-1}$,
%      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
  ]
  {\dataAnisoTwoDdegThree}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}
  \caption{2D case: dependency of the number of iterations of the Conjugate Gradient (CG) method and with symmetric block Gauss-Seidel preconditioner (PCG-GS) 
  %and with block-Jacobi preconditioner (PCG-J)) 
  w.r.t. the mesh parameter $L$, for the case with degree $p = 3$ and $n=2$ (i.e. $5$ overlapping domains).} \label{table:aniso_2D_deg3_n2}
\end{table}


\subsection{Case ???: 3D, polar mapping, anisotropic refinement}
For this case $d=3$ and $\Omega$ is the image of the parametric domain $$\widehat\Omega:=[1,2] \times [\frac{\pi}{4},\frac{3 \pi}{4}] \times [0,\frac{\pi}{2}]$$
 under the polar mapping $$ F(\rho,\theta,\phi) = \bigl( \rho \cos(\theta), \rho \sin(\theta) \cos(\phi),  \rho \sin(\theta) \sin(\phi) \bigr)^T.$$
The test and trial space $V$ is defined as $V = V_0 + \sum_{k=1}^n \bigl( V_k^{x} + V_k^{y} + V_k^{z} \bigr)$, where:
\begin{itemize}
  \item $V_0$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat\Omega$ with uniform knots vectors of size $\frac{1}{2^{L+2}} (1, \frac{\pi}{2}, \frac{\pi}{2})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The correspondent physical domain of this space is depicted in Fig.\ref{fig:3d_V0};
  \item $V_k^{x}$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat{\Omega}_k^x = [ 1,\frac{3}{2} ] \times [ \frac{\pi}{4},\frac{\pi}{4} \bigl( 1 + \frac{1}{2^{k-1}} \bigr) ] \times [0,\frac{\pi}{2^{k+1}}] $, with uniform knots vectors of size $\frac{1}{2^{L+2}} (1, \frac{\pi}{2^{k+1}}, \frac{\pi}{2^{k+1}})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The physical domains corresponding to the spaces $V_1^{x}$ and $V_2^{x}$  (with $L=0$) are depicted in Fig.\ref{fig:3d_V1x} and Fig.\ref{fig:3d_V2x}, respectively;
  \item $V_k^{y}$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat{\Omega}_k^y = [ 1,1 + \frac{1}{2^k} ] \times [ \frac{\pi}{4},\frac{5 \pi}{8} ] \times [ 0,\frac{\pi}{2^{k+1}} ]$, with uniform knots vectors of size $\frac{1}{2^{L+2}} (\frac{1}{2^k}, \frac{\pi}{2}, \frac{\pi}{2^{k+1}})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The physical domains corresponding to the spaces $V_1^{y}$ and $V_2^{y}$ (with $L=0$) are depicted in Fig.\ref{fig:3d_V1y} and Fig.\ref{fig:3d_V2y}, respectively;
  \item $V_k^{z}$ is the push forward through $F$ of the spline space of degree $p$ and continuity $p-1$, built over $\widehat{\Omega}_k^z = [ 1,1 + \frac{1}{2^k} ] \times [ \frac{\pi}{4},\frac{\pi}{4} \bigl( 1 + \frac{1}{2^{k-1}} \bigr) ] \times [ 0,\frac{3 \pi}{8} ]$ with uniform knots vectors of size $\frac{1}{2^{L+2}} (\frac{1}{2^k}, \frac{\pi}{2^{k+1}}, \frac{\pi}{2})$ (with $L \ge0$) and satisfying homogeneous Dirichlet boundary conditions. The physical domains corresponding to the spaces $V_1^{z}$ and $V_2^{z}$  (with $L=0$) are depicted in Fig.\ref{fig:3d_V1z} and Fig.\ref{fig:3d_V2z}, respectively.
\end{itemize}
Note that with this choice, the meshes related to $V_k^{x}$, $V_k^{y}$ and $V_k^{z}$ have the same number of elements, independently from $k$.

\begin{figure}
  \centering
  \includegraphics[width=.4\linewidth]{figures/plot_3d_00.png}
  \caption{3D case: the physical domain $F(\widehat{\Omega}_0)$ associated to the space $V_0$ for $L=0$.}
  \label{fig:3d_V0}
\end{figure}

\begin{figure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_x_liv1.png}
  \caption{$F(\widehat{\Omega}_{1,x})$}
  \label{fig:3d_V1x}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_x_liv2.png}
  \caption{$F(\widehat{\Omega}_{2,x})$}
  \label{fig:3d_V2x}
\end{subfigure}
\vfill
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_y_liv1.png}
  \caption{$F(\widehat{\Omega}_{1,y})$}
  \label{fig:3d_V1y}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_y_liv2.png}
  \caption{$F(\widehat{\Omega}_{2,y})$}
  \label{fig:3d_V2y}
\end{subfigure}%
\vfill
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_z_liv1.png}
  \caption{$F(\widehat{\Omega}_{1,z})$}
  \label{fig:3d_V1z}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.8\linewidth]{figures/plot_3d_z_liv2.png}
  \caption{$F(\widehat{\Omega}_{2,z})$}
  \label{fig:3d_V2z}
\end{subfigure}
\caption{3D case: the different physical domains associated to the spaces $V_{1}^x$ (\ref{fig:3d_V1x}), $V_{2}^x$ (\ref{fig:3d_V2x}), $V_{1}^y$ (\ref{fig:3d_V1y}), $V_{2}^y$ (\ref{fig:3d_V2y}), $V_{1}^z$ (\ref{fig:3d_V1z}) and $V_{2}^z$ (\ref{fig:3d_V2z}) for $L=0$.}
\label{fig:3d_phys_domains}
\end{figure}

We tested the proposed method with $n=2$ (corresponding to 7 overlapping domains) with different values of the mesh parameter $L$ for degrees $p=2$ (Table~\ref{table:aniso_3D_deg2_n2}) and $p=3$ (Table~\ref{table:aniso_3D_deg3_n2}), where can be observed that the use of the symmetric Gauss-Seidel preconditioner in the Conjugate Gradient solver gives us a substantial advantage (in term of number of required iterations) with respect to the strategy with no preconditioner. In the aformentioned tests we don't see (yet) the expected independence of the number of iterations with respect to the mesh parameter $L$, but this is due to the fact that the used meshes\footnote{Due to hardware limitations, we were not able to perform 3D simulation with finer meshes.} were too coarse to show this phenomena, that is clearly visible in the 2D tests (see Subsection~\ref{sec:test_2D_1}, Tables~\ref{table:aniso_2D_deg2_n2} and \ref{table:aniso_2D_deg3_n2}).

\pgfplotstableset{create on use/NewColL3D/.style={create col/set list={0,1,2,3},},columns/NewColL3D/.style={string type},}

%--------------------------------------------------------------------------------------------------------------
% 3D, degree=2
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_3D_anisotropic_2_deg_min=2_deg_max=2_nlevels_min=2_nlevels_max=2_polar_map_gauss_seidel.dat}{\dataAnisoThreeDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 11}
%]{13}{\dataAnisoTwoDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 12}
%]{14}{\dataAnisoTwoDdegTwo}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={NewColL3D,7,9,10,11,12},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/NewColL3D/.style={
      column name=$L$,
      int detect},
%    columns/1/.style={
%      column name=$h^{-1}$,
%      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
  ]
  {\dataAnisoThreeDdegTwo}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}
  \caption{3D case: dependency of the number of iterations of the Conjugate Gradient (CG) method and with symmetric block Gauss-Seidel preconditioner (PCG-GS) 
  %and with block-Jacobi preconditioner (PCG-J)) 
  w.r.t. the mesh parameter $L$, for the case with degree $p = 2$ and $n=2$ (i.e. $7$ overlapping domains).} \label{table:aniso_3D_deg2_n2}
\end{table}

%--------------------------------------------------------------------------------------------------------------
% 3D, degree=3
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_3D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_polar_map_gauss_seidel.dat}{\dataAnisoThreeDdegThree}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 11}
%]{13}{\dataAnisoTwoDdegTwo}
%\pgfplotstablecreatecol[
%  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 12}
%]{14}{\dataAnisoTwoDdegTwo}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={NewColL3D,7,9,10,11,12},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/NewColL3D/.style={
      column name=$L$,
      int detect},
%    columns/1/.style={
%      column name=$h^{-1}$,
%      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
  ]
  {\dataAnisoThreeDdegThree}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}
  \caption{3D case: dependency of the number of iterations of the Conjugate Gradient (CG) method and with symmetric block Gauss-Seidel preconditioner (PCG-GS) 
  %and with block-Jacobi preconditioner (PCG-J)) 
  w.r.t. the mesh parameter $L$, for the case with degree $p = 3$ and $n=2$ (i.e. $7$ overlapping domains).} \label{table:aniso_3D_deg3_n2}
\end{table}

\subsection{Case 1: 2D, identity mapping, anisotropic refinement} \label{sec:num_tests_1}

For this case $d=2$, $\Omega = [0,1] \times [0,1]$ (i.e. the physical domain coincides with the parametric domain), and the test and trial space $V$ is defined as $V = V_0 + \sum_{k=1}^n (V_k^{x} + V_k^{y})$, where:
\begin{itemize}
  \item $V_0$ is the space generated by the B-spline basis functions $\{ v_{0,i} \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_0 = [ 0,1 ] \times [ 0,1 ]$ spanned by uniform knots vectors of size $h$ and such that $v_{0,i} \vert_{\partial \widehat{\Omega}_0} = 0$;
  \item $V_k^{x}$ is the space generated by the B-spline basis functions $\{ v_{k,i}^x \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_k^x = [ 0,\frac{3}{4} ] \times [ 0,2^{-k} ]$ spanned by uniform knots vectors of size $(h,\frac{h}{2^k})$ and such that $v_{k,i}^x \vert_{\partial \widehat{\Omega}_k^x} = 0$;
  \item $V_k^{y}$ is the space generated by the B-spline basis functions $\{ v_{k,i}^y \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_k^y = [ 0,2^{-k} ] \times [ 0,\frac{3}{4} ]$ spanned by uniform knots vectors of size $(\frac{h}{2^k},h)$ and such that $v_{k,i}^y \vert_{\partial \widehat{\Omega}_k^y} = 0$.
\end{itemize}
Note that with this choice, the meshes related to $V_k^{x}$ and $V_k^{y}$ have the same number of elements, independently from $k$.

In Figure~\ref{fig:meshes_2D_1} is shown an example of space configuration for $h=\frac{1}{4}$ and $n=0,\dots,3$.

\begin{figure}
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \draw (0,1) -- (4,1);
      \draw (0,2) -- (4,2);
      \draw (0,3) -- (4,3);
      \draw (1,0) -- (1,4);
      \draw (2,0) -- (2,4);
      \draw (3,0) -- (3,4);
    \end{tikzpicture}
    \subcaption{$n=0$}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \draw (0,1) -- (4,1);
      \draw (0,2) -- (4,2);
      \draw (0,3) -- (4,3);
      \draw (1,0) -- (1,4);
      \draw (2,0) -- (2,4);
      \draw (3,0) -- (3,4);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,2);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (2,3);

      \draw (0,0.5) -- (3,0.5);
      \draw (0,1.5) -- (3,1.5);

      \draw (0.5,0) -- (0.5,3);
      \draw (1.5,0) -- (1.5,3);
    \end{tikzpicture}
    \subcaption{$n=1$}
  \end{minipage}
  \begin{minipage}[b]{0.5\textwidth}
    \vspace{1cm}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \draw (0,1) -- (4,1);
      \draw (0,2) -- (4,2);
      \draw (0,3) -- (4,3);
      \draw (1,0) -- (1,4);
      \draw (2,0) -- (2,4);
      \draw (3,0) -- (3,4);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,2);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (2,3);

      \draw (0,0.5) -- (3,0.5);
      \draw (0,1.5) -- (3,1.5);

      \draw (0.5,0) -- (0.5,3);
      \draw (1.5,0) -- (1.5,3);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,1);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (1,3);

      \draw (0,0.25) -- (3,0.25);
      \draw (0,0.75) -- (3,0.75);

      \draw (0.25,0) -- (0.25,3);
      \draw (0.75,0) -- (0.75,3);
    \end{tikzpicture}
    \subcaption{$n=2$}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.5\textwidth}
    \vspace{1cm}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \draw (0,1) -- (4,1);
      \draw (0,2) -- (4,2);
      \draw (0,3) -- (4,3);
      \draw (1,0) -- (1,4);
      \draw (2,0) -- (2,4);
      \draw (3,0) -- (3,4);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,2);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (2,3);

      \draw (0,0.5) -- (3,0.5);
      \draw (0,1.5) -- (3,1.5);

      \draw (0.5,0) -- (0.5,3);
      \draw (1.5,0) -- (1.5,3);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,1);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (1,3);

      \draw (0,0.25) -- (3,0.25);
      \draw (0,0.75) -- (3,0.75);

      \draw (0.25,0) -- (0.25,3);
      \draw (0.75,0) -- (0.75,3);

      \draw [fill=red, fill opacity=.25] (0,0) rectangle (3,0.5);
      \draw [fill=blue, fill opacity=.25] (0,0) rectangle (0.5,3);

      \draw (0,0.125) -- (3,0.125);
      \draw (0,0.375) -- (3,0.375);

      \draw (0.125,0) -- (0.125,3);
      \draw (0.375,0) -- (0.375,3);
    \end{tikzpicture}
    \subcaption{$n=3$}
  \end{minipage}
  \caption{Example of space configuration for the case described in Section~\ref{sec:num_tests_1} with $h=\frac{1}{4}$ and $n=0,\dots,3$.} \label{fig:meshes_2D_1}
\end{figure}

In the Tables~\ref{table:aniso_2D_n2}--\ref{table:aniso_2D_n5} is shown the dependency of the number of iterations of the Conjugate Gradient (CG) method and Preconditioned Conjugate Gradient (PCG) method (both with with symmetric block Gauss-Seidel (PCG-GS) preconditioner and block Jacobi preconditioner (PCG-J)) w.r.t. the mesh size $h$, for the case with degree $p = 3$. Table~\ref{table:aniso_2D_n2} refers to the case with $n=2$ (i.e. 5 overlapping domains), while Table~\ref{table:aniso_2D_n5} refers to the case with $n=5$ (i.e. 11 overlapping domains). From the data we can observe that...\marginpar{Completare}


% \begin{tikzpicture}
% %  	\draw[black, line width=1pt] (0,0) grid[step=1] (4,4);
%   	\draw[black, line width=1pt, step=5mm] (0,0) grid (4,4);
% \end{tikzpicture}
%
% \begin{tikzpicture}
%   	\draw[black, line width=1pt, xstep=5mm, ystep=2.5mm] (0,0) grid (3,2);
% \end{tikzpicture}

\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}{\dataAnisoTwoDdegTwo}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 11}
]{13}{\dataAnisoTwoDdegTwo}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_jacobi.dat}{[index] 12}
]{14}{\dataAnisoTwoDdegTwo}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={1,7,9,10,11,12,13,14},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/1/.style={
      column name=$h^{-1}$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataAnisoTwoDdegTwo}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=2_nlevels_max=2_identity_map_gauss_seidel.dat}
  \caption{Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) methods (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the mesh size $h$, for the case with degree $p = 3$ and $n=2$ (i.e. $5$ overlapping domains).} \label{table:aniso_2D_n2}
\end{table}



\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=5_nlevels_max=5_identity_map_gauss_seidel.dat}{\dataAnisoTwoDNFive}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=5_nlevels_max=5_identity_map_jacobi.dat}{[index] 11}
]{13}{\dataAnisoTwoDNFive}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=5_nlevels_max=5_identity_map_jacobi.dat}{[index] 12}
]{14}{\dataAnisoTwoDNFive}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={1,7,9,10,11,12,13,14},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/1/.style={
      column name=$h^{-1}$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataAnisoTwoDNFive}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=5_nlevels_max=5_identity_map_gauss_seidel.dat}
  \caption{Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) methods (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the mesh size $h$, for the case with degree $p = 3$ and $n=5$ (i.e. $11$ overlapping domains).} \label{table:aniso_2D_n5}
\end{table}


The Table~\ref{table:aniso_2D_h32} refers to the case with degree $p = 3$ and initial mesh size $h=\frac{1}{32}$, and shows the dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) method (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the parameter $n$ (equivalent to $2n+1$ overlapping patches). From the data we can observe that...\marginpar{Completare}



\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=10_identity_map_gauss_seidel.dat}{\dataAnisoTwoDhFixed}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=10_identity_map_jacobi.dat}{[index] 11}
]{13}{\dataAnisoTwoDhFixed}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=10_identity_map_jacobi.dat}{[index] 12}
]{14}{\dataAnisoTwoDhFixed}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={2,7,9,10,11,12,13,14},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/2/.style={
      column name=$n$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataAnisoTwoDhFixed}
%  {./numerical_tests/convergence_results_2D_anisotropic_2_deg_min=3_deg_max=3_nlevels_min=5_nlevels_max=5_identity_map_gauss_seidel.dat}
  \caption{
%  Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) methods (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the mesh size $h$, for the case with degree $p = 3$ and $n=5$ (i.e. $11$ overlapping domains).
  Degree $p = 3$ and initial mesh size $h=\frac{1}{32}$. Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) method (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the parameter $n$ (equivalent to $2n+1$ overlapping patches).}
  \label{table:aniso_2D_h32}
\end{table}

%\subsection{X-FEM refinement}\label{ex:xfem}

\subsection{Diagonal refinement (overlap 1)} %\label{ex:diagonal_overlap_1}
\label{sec:diagonal_overlap_1}
$V = V_0 + \sum_{k=1}^n \sum_{j=0}^{2(2^k-1)} V_{k,j}$

\begin{itemize}
  \item $V_0$ is the space generated by the B-spline basis functions $\{ v_{0,i} \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_0 = [ 0,1 ] \times [ 0,1 ]$ spanned by uniform knots vectors of size $h_0 = \frac{1}{2(p+1)}$ and such that $v_{0,i} \vert_{\partial \widehat{\Omega}_0} = 0$;
  \item $V_{k,j}$ ($j=0,\dots,2(2^k-1)$) is the space generated by the B-spline basis functions $\{ v_{k,j,i} \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_{k,j} = [ \frac{j}{2^{k+1}},\frac{j}{2^{k+1}} ] \times [ \frac{j+2}{2^{k+1}},\frac{j+2}{2^{k+1}} ]$ spanned by uniform knots vectors of size $h_k = \frac{h_0}{2^k}$ and such that $v_{k,j,i} \vert_{\partial \widehat{\Omega}_{k,j}} = 0$.
\end{itemize}

With the previous definitions:
\begin{itemize}
  \item the domain $\widehat{\Omega}_{k,j}$ fully supports one basis function from the coarser space $V_{k-1,???}$;  \marginpar{sistemare il secondo indice}
  \item the domain $\widehat{\Omega}_{k,j} \cap \widehat{\Omega}_{k,j+1} = \bigl[ \frac{j+1}{2^{k+1}},\frac{j+1}{2^{k+1}} \bigr] \times \bigl[ \frac{j+2}{2^{k+1}},\frac{j+2}{2^{k+1}} \bigr]$ fully supports only one basis function from the space $V_{k,j}$ and one from the space $V_{k,j+1}$, therefore the overlap of the spaces $V_{k,j}$ and $V_{k,j+1}$ is ``minimal''.
\end{itemize}

\begin{figure}
  \def \p {2}
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }
    \end{tikzpicture}
    \subcaption{$n=0$}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }

      \foreach \j in {0,...,2} {
        \def \xmin {4 * \j / 4}
        \def \xmax {\xmin + 2}
        \draw [fill=red, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
      }

      \foreach \i in {1,3,5} {
        \def \j {\i / 3}
        \draw (0,\j) -- (2,\j);
        \draw (\j,0) -- (\j,2);
      }

      \foreach \i in {5,7} {
        \def \j {\i / 3}
        \draw (1,\j) -- (3,\j);
        \draw (\j,1) -- (\j,3);
      }

      \foreach \i in {7,9,11} {
        \def \j {\i / 3}
        \draw (2,\j) -- (4,\j);
        \draw (\j,2) -- (\j,4);
      }
    \end{tikzpicture}
    \subcaption{$n=1$}
  \end{minipage}
  \begin{minipage}[b]{0.5\textwidth}
    \vspace{1cm}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }


      \foreach \j in {0,...,2} {
        \def \xmin {4 * \j / 4}
        \def \xmax {\xmin + 2}
        \draw [fill=red, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
      }

      \foreach \i in {1,3,5} {
        \def \j {\i / 3}
        \draw (0,\j) -- (2,\j);
        \draw (\j,0) -- (\j,2);
      }

      \foreach \i in {5,7} {
        \def \j {\i / 3}
        \draw (1,\j) -- (3,\j);
        \draw (\j,1) -- (\j,3);
      }

      \foreach \i in {7,9,11} {
        \def \j {\i / 3}
        \draw (2,\j) -- (4,\j);
        \draw (\j,2) -- (\j,4);
      }


      \foreach \j in {0,...,6} {
        \def \xmin {4 * \j / 8}
        \def \xmax {\xmin + 1}
        \draw [fill=blue, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
      }

      \foreach \i in {1,3,5} {
        \def \j {\i / 6}
        \draw (0,\j) -- (1,\j);
        \draw (\j,0) -- (\j,1);
      }

      \foreach \i in {5,7} {
        \def \j {\i / 6}
        \draw (0.5,\j) -- (1.5,\j);
        \draw (\j,0.5) -- (\j,1.5);
      }

      \foreach \i in {7,9,11} {
        \def \j {\i / 6}
        \draw (1,\j) -- (2,\j);
        \draw (\j,1) -- (\j,2);
      }

      \foreach \i in {11,13} {
        \def \j {\i / 6}
        \draw (1.5,\j) -- (2.5,\j);
        \draw (\j,1.5) -- (\j,2.5);
      }

      \foreach \i in {13,15,17} {
        \def \j {\i / 6}
        \draw (2,\j) -- (3,\j);
        \draw (\j,2) -- (\j,3);
      }

      \foreach \i in {17,19} {
        \def \j {\i / 6}
        \draw (2.5,\j) -- (3.5,\j);
        \draw (\j,2.5) -- (\j,3.5);
      }

      \foreach \i in {19,21,23} {
        \def \j {\i / 6}
        \draw (3,\j) -- (4,\j);
        \draw (\j,3) -- (\j,4);
      }

    \end{tikzpicture}
    \subcaption{$n=2$}
  \end{minipage}
  \caption{Example of space configuration for the case described in Section~\ref{sec:diagonal_overlap_1} with $p=2$ (i.e. $h_0=\frac{1}{6})$ and $n=0,\dots,2$.} \label{fig:meshes_2D_overlap_1}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=9_identity_map_gauss_seidel.dat}{\dataDiagonalTwoDidentityMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=9_identity_map_jacobi.dat}{[index] 11}
]{13}{\dataDiagonalTwoDidentityMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=9_identity_map_jacobi.dat}{[index] 12}
]{14}{\dataDiagonalTwoDidentityMap}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={2,7,9,10,11,12,13,14},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/2/.style={
      column name=$n$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataDiagonalTwoDidentityMap}
  \caption{
  Diagonal overlap 1, identity map (see Section~\ref{sec:diagonal_overlap_1}) with degree $p=3$.
  Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) method (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the parameter $n$.}
  \label{table:diagonal_2D_identity_map}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=7_polar_map_gauss_seidel.dat}{\dataDiagonalTwoDpolarMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=7_polar_map_jacobi.dat}{[index] 11}
]{13}{\dataDiagonalTwoDpolarMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=7_polar_map_jacobi.dat}{[index] 12}
]{14}{\dataDiagonalTwoDpolarMap}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={2,7,9,10,11,12,13,14},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/2/.style={
      column name=$n$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataDiagonalTwoDpolarMap}
  \caption{
  Diagonal overlap 1, polar map (see Section~\ref{sec:diagonal_overlap_1}) with degree $p=3$.
  Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) method (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the parameter $n$.}
  \label{table:diagonal_2D_polar_map}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





\subsection{Diagonal refinement (overlap $(p+1) \times (p+1)$)}\label{ex:diagonal_overlap_p_plus_1}

\label{sec:diagonal_overlap_p_plus_1}
$V = V_0 + \sum_{k=1}^n \sum_{j=0}^{2(p+1)(2^k-1)} V_{k,j}$

\begin{itemize}
  \item $V_0$ is the space generated by the B-spline basis functions $\{ v_{0,i} \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_0 = [ 0,1 ] \times [ 0,1 ]$ spanned by uniform knots vectors of size $h_0 = \frac{1}{2(p+1)}$ and such that $v_{0,i} \vert_{\partial \widehat{\Omega}_0} = 0$;
  \item $V_{k,j}$ ($j=0,\dots,2(p+1)(2^k-1)$) is the space generated by the B-spline basis functions $\{ v_{k,j,i} \}_{i}$  of degree $p$ and continuity $p-1$, over the two-dimensional parametric domain $\widehat{\Omega}_{k,j} = [ \frac{j h_0}{2^{k}},\frac{j h_0}{2^{k}} ] \times [ \frac{j h_0 + 1}{2^{k}},\frac{j h_0 + 1}{2^{k}} ]$ spanned by uniform knots vectors of size $h_k = \frac{h_0}{2^k}$ and such that $v_{k,j,i} \vert_{\partial \widehat{\Omega}_{k,j}} = 0$.
\end{itemize}

With the previous definitions the domain $\widehat{\Omega}_{k,j} \cap \widehat{\Omega}_{k,j+1} = [ \frac{(j+1) h_0}{2^{k}},\frac{(j+1) h_0}{2^{k}} ] \times [ \frac{j h_0 + 1}{2^{k}},\frac{j h_0 + 1}{2^{k}} ]$ fully supports $(p+1) \times (p+1)$ basis function from the space $V_{k,j}$ and from the space $V_{k,j+1}$.


\begin{figure}
  \def \p {2}
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }
    \end{tikzpicture}
    \subcaption{$n=0$}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\textwidth}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }

      \foreach \j in {0,...,6} {
        \def \xmin {\j / 3}
        \def \xmax {\xmin + 2}
        \draw [fill=red, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
        \foreach \i in {1,...,5} {
          \def \v {\xmin + \i/3}
          \draw (\v,\xmin) -- (\v,\xmax);
          \draw (\xmin,\v) -- (\xmax,\v);
        }
      }

    \end{tikzpicture}
    \subcaption{$n=1$}
  \end{minipage}
  \begin{minipage}[b]{0.5\textwidth}
    \vspace{1cm}
    \centering
    \begin{tikzpicture}
      \draw (0,0) rectangle (4,4);
      \foreach \i in {1,...,5} {
        \def \j {\i / 1.5}
        \draw (0,\j) -- (4,\j);
        \draw (\j,0) -- (\j,4);
      }

      \foreach \j in {0,...,6} {
        \def \xmin {\j / 3}
        \def \xmax {\xmin + 2}
        \draw [fill=red, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
        \foreach \i in {1,...,5} {
          \def \v {\xmin + \i/3}
          \draw (\v,\xmin) -- (\v,\xmax);
          \draw (\xmin,\v) -- (\xmax,\v);
        }
      }

      \foreach \j in {0,...,18} {
        \def \xmin {\j / 6}
        \def \xmax {\xmin + 1}
        \draw [fill=blue, fill opacity=.25] (\xmin,\xmin) rectangle (\xmax,\xmax);
        \foreach \i in {1,...,5} {
          \def \v {\xmin + \i / 6}
          \draw (\v,\xmin) -- (\v,\xmax);
          \draw (\xmin,\v) -- (\xmax,\v);
        }
      }


    \end{tikzpicture}
    \subcaption{$n=2$}
  \end{minipage}
  \caption{Example of space configuration for the case described in Section~\ref{sec:diagonal_overlap_p_plus_1} with $p=2$ (i.e. $h_0=\frac{1}{6})$ and $n=0,\dots,2$.} \label{fig:meshes_2D_overlap_p+plus_1}
\end{figure}


\pgfplotstableread[skip first n=1]{./numerical_tests/convergence_results_2D_diagonal_max_overlap_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=8_identity_map_gauss_seidel.dat}{\dataDiagonalMaxOverlapTwoDidentityMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_max_overlap_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=8_identity_map_jacobi.dat}{[index] 11}
]{13}{\dataDiagonalMaxOverlapTwoDidentityMap}
\pgfplotstablecreatecol[
  create col/copy column from table={./numerical_tests/convergence_results_2D_diagonal_max_overlap_deg_min=3_deg_max=3_nlevels_min=1_nlevels_max=8_identity_map_jacobi.dat}{[index] 12}
]{14}{\dataDiagonalMaxOverlapTwoDidentityMap}


\begin{table}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={2,7,9,10,11,12,13,14},
%    columns={2,7,9,10,11,12},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG-GS} & \multicolumn{2}{c}{PCG-J} \\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    sci zerofill,
    precision=2,
    columns/2/.style={
      column name=$n$,
      int detect},
    columns/7/.style={
      column name=DOFs,
      int detect},
    columns/9/.style={
      column name=N. iters,
      int detect
%      ,column type/.add={|}{}
      }, % N.iters CG
    columns/10/.style={
      column name=Residual}, % residual CG
    columns/11/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-GS
    columns/12/.style={
      column name=Residual}, % residual PCG-GS
    columns/13/.style={
      column name=N. iters,
      int detect}, % N.iters PCG-J
    columns/14/.style={
      column name=Residual}, % residual PCG-J
  ]
  {\dataDiagonalMaxOverlapTwoDidentityMap}
  \caption{
  Diagonal overlap $p+1$ (see Section~\ref{ex:diagonal_overlap_p_plus_1}) with degree $p=3$.
  Dependency of the number of iterations of the Conjugate Gradient (CG) method and two Preconditioned Conjugate Gradient (PCG) method (with symmetric block Gauss-Seidel preconditioner (PCG-GS) and with block-Jacobi preconditioner (PCG-J)) w.r.t. the parameter $n$.}
  \label{table:diagonal_2D_overlap_p_plus1_identity_map}
\end{table}


==> numerical-examples_old.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex

\section{Numerical examples}

\subsection{Local refinement}\label{ex:local-refinement}

\subsection{Anisotropic refinement}\label{ex:anisotropic-refinement}





\begin{tikzpicture}
%  	\draw[black, line width=1pt] (0,0) grid[step=1] (4,4);
  	\draw[black, line width=1pt, step=5mm] (0,0) grid (4,4);
\end{tikzpicture}

\begin{tikzpicture}
  	\draw[black, line width=1pt, xstep=5mm, ystep=2.5mm] (0,0) grid (3,2);
\end{tikzpicture}




\begin{figure}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={0,5,7,8,9,10},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG}\\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    columns/0/.style={
      column name=$N_h$,
      int detect},
    columns/5/.style={
      column name=DOFs,
      int detect},
    columns/7/.style={
      column name=N. iters,
      int detect}, % N.iters CG
    columns/8/.style={
      column name=residual}, % residual CG
    columns/9/.style={
      column name=N. iters,
      int detect}, % N.iters PCG
    columns/10/.style={
      column name=residual} % residual PCG
  ]{../../risultati_igatools/2D/anisotropic_2/convergence_results_anisotropic_2_deg=2_nlevels=1_2D.dat}
  \caption{Degree $p=2$.}
\end{figure}


\begin{figure}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={0,5,7,8,9,10},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG}\\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    columns/0/.style={
      column name=$N_h$,
      int detect},
    columns/5/.style={
      column name=DOFs,
      int detect},
    columns/7/.style={
      column name=N. iters,
      int detect}, % N.iters CG
    columns/8/.style={
      column name=residual}, % residual CG
    columns/9/.style={
      column name=N. iters,
      int detect}, % N.iters PCG
    columns/10/.style={
      column name=residual} % residual PCG
  ]{../../risultati_igatools/2D/anisotropic_2/convergence_results_anisotropic_2_deg=3_nlevels=1_2D.dat}
  \caption{Degree $p=3$.}
\end{figure}


\begin{figure}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={0,5,7,8,9,10},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG}\\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    columns/0/.style={
      column name=$N_h$,
      int detect},
    columns/5/.style={
      column name=DOFs,
      int detect},
    columns/7/.style={
      column name=N. iters,
      int detect}, % N.iters CG
    columns/8/.style={
      column name=residual}, % residual CG
    columns/9/.style={
      column name=N. iters,
      int detect}, % N.iters PCG
    columns/10/.style={
      column name=residual} % residual PCG
  ]{../../risultati_igatools/2D/anisotropic_2/convergence_results_anisotropic_2_deg=4_nlevels=1_2D.dat}
  \caption{Degree $p=4$.}
\end{figure}


\begin{figure}
  \centering
  \pgfplotstabletypeset[
    skip first n=1,
    columns={0,5,7,8,9,10},
    every head row/.style={
      before row={
      \toprule
      & & \multicolumn{2}{c}{CG} & \multicolumn{2}{c}{PCG}\\
      },
      after row=\midrule,
    },
    every last row/.style={
      after row=\bottomrule},
    columns/0/.style={
      column name=$N_h$,
      int detect},
    columns/5/.style={
      column name=DOFs,
      int detect},
    columns/7/.style={
      column name=N. iters,
      int detect}, % N.iters CG
    columns/8/.style={
      column name=residual}, % residual CG
    columns/9/.style={
      column name=N. iters,
      int detect}, % N.iters PCG
    columns/10/.style={
      column name=residual} % residual PCG
  ]{../../risultati_igatools/2D/anisotropic_2/convergence_results_anisotropic_2_deg=5_nlevels=1_2D.dat}
  \caption{Degree $p=5$.}
\end{figure}


\subsection{X-FEM refinement}\label{ex:xfem}

\subsection{Diagonal refinement}\label{ex:diagonal}




==> old-removed.tex <==
\section{old removed}

\subsection{Geometric interpretation}
Assume that the \(R_i\) are the exact solver for the Galerkin problem
\[
    a(R_i v, w_i)=a(v,w_i), \,\qquad\forall w_i\in V_i.
\]
Then \(T_i\) is the \(a\)-orthogonal projection \(V\to V_i\) as it
preserve all scalar products.
Thus \(\Tp\) associates to each \(v\in V\) the sum of its projections on the \(V_i\),
and \(\Ts\) associates to each \(v\) the difference between \(v\) and the composition
of the projection on the orthogonal complement of the \(V_i\).

Clearly the properties of these operations in \(a\)-norm are determined by the geometric
properties of the collection of the spaces \(V_i\), in particular on the angles
measured in the \(a\) scalar product.
Indeed let \( \C_{\min} \) be the minimum cosine between a vector \(v\in V\) and the \(V_i\):
\[
    \C_{\min}:= \inf_{v\ne 0 \in V}\max_i \sup_{w_i\ne 0\in V_i} \frac{a(v,w_i)}{\n{w_i}_a \n{v}_a}
\]
The best possible bound on 

\begin{lem}\label{thm:S-inverse-norm}
    For all \(v\in V\) there is \(\wv\in S^{-1}v \) satisfying 
\[
    \n{\wv}_\wA\le \frac\rho{1-\rho}\n{v}_A.
\]
and \(\rho=\sqrt{1-\C_{\min}^2}\).

\end{lem}

\begin{proof}
For all \(v\in V\) 
\[
    \n{v}_a^2=\n{T_i v}_a^2 + \n{v-T_i v}_a^2
\]
so that by choosing \(i\) that maximize \(\n{T_i v}_a^2\) we have
\[
    \n{v-T_i v}_a^2\le (1-\C_{\min}^2)\n{v}_a^2 \quad\thus\quad \n{v-T_i v}_a\le\rho\n{v}_a.
\]
Then starting from \(v\in V\) we build \(\wv\) as the limit of
\(\wBs^{[k]} S^* A v\) where \(\wBs^{[k]}\) corresponds to the \(v\) dependent 
sequence of steps \(i_1,\dots,i_k\) with the property that at each step
the norm of \( \n{T_{i_j}\wBs^{[j-1]} S^* A v S v}_a^2 \) is maximized.

It follows that \(\n{v-\wBs^{[k]} S^* A v}_a\le \rho^k \) and 
\[
\n{\wv}_a= \n{\sum_{j} \wT_{i_j} (\Id-\wBs^{[j-1]} S^* A) v }_a\le \sum_{j=1}^{\infty} \rho^j.
\]
\end{proof}

Lemma~\ref{thm:S-inverse-norm} highlights how the existence of
stable decompositions is related to how well the \(V_i\) cover 
all directions in \(V\).
The following example in 2D shows that if some 







Let \(\C_{i,j}\) be the cosine between \(V_i\) and \(V_j\)
\[
\C_{i,j}:=\sup_{\substack{u_i\in V_i\\v_j\in V_j}} \frac{a(u_i,v_j)}{\n{u_i}_a \n{v_j}_a}\le 1.
\]
Then the matrix \(\C_{i,j}\) is the identity if and only if the \(V_i\)
are mutually \(a\)-orthogonal, so that \(\C_{i,j}\) ``measures'' the redundancy
of the generating set \(\wPhi\).
In particular,it gives an easy upper bound on the norm of \(\Tp\) as
\[
\n{\Tp S \wv}_a=\n{\sum_i T_i S\wv}_a=\n{\sum_{i,j} T_i v_j}_a 
\]

\[
\begin{aligned}
    a(S\wTp\wu,S\wTp\wv)&\le \sum_{i,j} \C_{i,j} \n{T_i u_i}_a \n{ T_j v_j}_a 
    \\ &\le  \Big(\sum_{i,j} \C_{i,j} a(T_i v_i, v_i)\Big)^{1/2} \Big(\sum_{j=1}^n a(T_j u_j, u_j)\Big)^{1/2}
\end{aligned}
\]
because the so that by

so that the strengthened Cauchy-Schwarz inequality holds with 
\[
    K_1=\max_i \sum_j \C_{i,j}.
\]

\(K_1\)







\[
\omega_1^2 \sum_{i,j} \C_{i,j}   \n{u_i}_V \n{v_j}_V
\\\le \omega_1^2 m \sum_i  \n{u_i}_V \Big( \sum_j \n{v_j}_V\Big)
\\ \le \omega_1^2 m \Big(\sum_i  \n{u_i}_V^2\Big)^{1/2} \Big( \sum_j \n{v_j}_V^2\Big)^{1/2}
\]


Then Lemma~\ref{thm:S-inverse-norm} gives an upper-bound for \(K_0\) in the stable decomposition in the simple terms of 
\[
    K_0\le \frac{\rho}{1-\rho} \omega_0. 
\]

Similarly \(K_1\) can be estimated in terms of properties of the \(V_i\) and \(\omega_1\).
Let
\[
\C_{i,j}:=\sup_{\substack{u_i\in V_i\\v_j\in V_j}} \frac{a(u_i,v_j)}{\n{u_i}_a \n{v_j}_a}\le 1,
\]
and \(m\) be
\[
    m:=\max_{i=1}^n \sum_j E_{i,j} \le \max_{i=1}^n \# \{j:E_{i,j}\ne 0\}.
\]
Intuitively \(E_{i,j}\) is the maximum \(cos\) between two vectors in the spaces \(V_i\) and \(V_j\) respectively and it \(1\) when the two spaces intersect.
Then for \(\wu=(u_1,\dots,u_n)\), \(\wv=(v_1,\dots,v_n)\) we have
\[
    \begin{aligned}
a(S\wT_p\wu,S\wT_p\wv)&\le \sum_{i,j} \C_{i,j} \n{R_iA_i u_i}_V \n{ R_jA_j v_j}_V \le \omega_1 \sum_{i,j} \C_{i,j}   \n{u_i}_V \n{v_j}_V
\\&\le \omega_1 m \sum_i  \n{u_i}_V \Big( \sum_j \n{v_j}_V\Big)
\\& \le \omega_1 m \Big(\sum_i  \n{u_i}_V^2\Big)^{1/2} \Big( \sum_j \n{v_j}_V^2\Big)^{1/2}
    \end{aligned}
\]
and 
\[
K_1\le m \omega_1.
\]
Note that if the spaces \(V_1,\dots,V_n\) are orthogonal then \(E_{i,j}\) is the identity matrix and \(K_1=\omega_1\).

Finally if \(R_i=A_i^{-1}\) and again with \(\n{\cdot}_V=\n{\cdot}_a\),the constants \(K_0\) and \(K_1\) are determined by the subspaces \(V_1,\dots,V_n\) and are the best constants for which the following ``(semi)-norm equivalency'' holds:  for all \(v\in V\),
\begin{equation}\label{eq:exact-inverse}
\begin{aligned}
&\forall \wv=(v_1,\dots,v_n)\in S^{-1} v, &&\n{v}_V^2 \le K_1\n{\wv}_\wV^2,
\\&\exists \wv'=(v_1',\dots,v_n')\in S^{-1} v: & K_0^{-1} \n{\wv'}_\wV^2 \le &\n{v}_V^2.
\end{aligned}
\end{equation}




In the elliptic case the general results admit a more intuitive interpretation.




Moreover if \(A\) is symmetric and positive definite then
\[
\inf_{\wv\in S^{-1} v} \sum_{i=1}^n (T_i v_i,v_i)_V = (T v,v)_V.
\]



\subsection{Some notes on the norm of \(S^{-1}_R\)}

The minimal norm of the right inverses \(S^{-1}_R\) of \(S\) is very important in the analysis \emph{subspace correction methods}, and it is often referred to as \emph{stable decompositions}.
Indeed a right-inverse of \(S\) is a map \(V\rightarrow \wV\) that associate to \(v\) a decomposition of \(v\) as a vector \(\wv=(v_1,\dots,v_n)\in \wV\) for which 
\[
    v=S\wv=\sum_{i=1}^n v_i.
\]
The norm of is minimized by choosing \(S^{-1}_R\) as the projection of a pre-image onto the orthogonal complement of \(\ker S\)
\[
    S^{-1}_R v= (\wId -\Pi^\perp_{\ker S} )S^{-1}v.
\]

The minimal norm can be characterized as a function of the geometry of the subspaces \(V_i\).

\begin{lem}%\label{thm:S-inverse-norm}
    There exists a nonlinear operator \(S^{-1}_{R,nl}\) with norm bounded by
    \[
        \n{S^{-1}_R} \le \frac{\rho}{1-\rho}
    \]    
    where
    \[
        \rho=\sup_{\substack{v\in V\\i=1,\dots,n}} \frac{\n{v}_V}{\n{v-\Pi^\perp_{V_i} v}_V}.
    \]
\end{lem}

\begin{proof}
    Let assume that \(\n{v}_V=1\), we build a sequence of \(\{\wv^{(j)}\}\) converging to a point in \(S^{-1}v\) using a non-linear version of SSC.
    At each step the correction is done on the subspace for which the norm of the correction is maximal.
    Let \(\wv^{(0)}=\w0\) and define 
    \[
        \wv^{(j+1)}=\wv^{(j)} + M_{s_j}(v-S\wv^{(j)})
    \]
    where 
    \[
        M_k(x)= (0,\dots,\Pi^\perp_{V_k}x,\dots,0)    
    \]
    and \(s_j\) is in \(\argmax\) of \(\n{M_k(v-S\wv^{(j)})}_\wV\).
   At each step
    \[ \n{v-S\wv^{(j+1)}}_V^2\le \rho^2 \n{v-S\wv^{(j)}}_V^2,\]
    and
    \[
        \n{ M_{s_j}(v-S\wv^{(j)})}_\wV=\n{\Pi^\perp_{V_{s_j}}(v-S\wv^{(j)})}_V^2 \le \n{v-S\wv^{(j)}}_V.
    \]
    Thus we have \[\lim_{j\to\infty} \n{v-S\wv^{(j)}}_V^2=0\] and 
    \[
        \lim_{j\to\infty}   \n{\wv^{(j)}}_\wV \le \lim_{j\to\infty}\sum_{k=1}^j \n{ M_{s_j}(v-S\wv^{(j)})}_\wV\le \sum_{j=1}^\infty \rho^j= \frac{\rho}{1-\rho}.
    \]
\end{proof}

The norm ratio \( \n{v-\Pi^\perp_{V_i} v}_V / \n{v}_V \) is the \(\sin\) of the angle between \(v\) and the space \(V_i\). The Lemma then states that to have stable decompositions, for any \(v\in V\) there should be a space \(V_i\) that is sufficiently far from orthogonal from \(v\).
In particular the problem is the representation of vectors of \(V\) and not the redundancy in \(\wV\) as it is shown by the following example in \(\R^2\).

\begin{example}
Let \(V=\R^2\) with the usual norm and let \(V_1=\SPAN\{(1,t)\}\), \(V_2=\SPAN\{(1,-t)\}\).
Then for \(t\ne0\), \(S\) is one to one so that 
\[
S^{-1}\begin{pmatrix}x\\y\end{pmatrix} = \left(\frac{y+tx}{2t}\begin{pmatrix}1\\t\end{pmatrix},\ \frac{tx-y}{2t}\begin{pmatrix}1\\-t\end{pmatrix}\right).
\]
Thus 
\[
	\n{S^{-1}(x,y)}_{\wV}=\sqrt{1+t^2}\frac{\sqrt{|y+tx|^2+|y+tx|^2}}{2t},
\]
and, in particular, that of \((0,1)\) is 
\[
	\frac{\sqrt{1+t^2}}{2t}=\frac12 (\sin\theta )^{-1}
\]
where \(\theta\) is the angle between \(V_1\) and \(V_2\). 
This means that as \(V_1\) and \(V_2\) become close to parallel the norm of \(S^{-1}\) goes to \(+\infty\). When \(t=0\) then the two spaces coincide and the norm of \(S^{-1}\) is 1. 

\begin{tikzpicture}[scale=1.5]
    \draw(-3,-.8)--(3,.8) node[above] {\(V_1\)}
            (3,-.8)--(-3,.8) node[above] {\(V_1\)};
    \draw[->] (0,0)--(2.25,.6) node[left] {\(v_1\)};
    \draw[->] (0,0)--(-2.25,.6) node[left] {\(v_2\)};
    \draw[dashed] (-2.25,.6) --(0,1.2) -- (2.25,.6);
    \draw[->] (0,0)--(0,1.2) node[above] {\(v\)};
    \draw[dotted] (0,1.2)--(.344,.092) node[right] {\(\Pi^\perp_{V_1} v\)};
    \draw[dotted] (0,1.2)--(-.344,.092) node[left] {\(\Pi^\perp_{V_2} v\)};
    %\draw[dotted] (.172,.046)--(-.172,.046) ;
    \draw[fill=red,red] (0,.046) circle(.5pt) node[above] {\(T v\)};
\end{tikzpicture}
\end{example}

Note that the sum of Hilbert spaces is not necessarily an Hilbert space because it can be incomplete, i.e. non-closed. 
The standard example is to take
\[
	V_1:=\SPAN\{e_{2i-1}+i^{-1}e_{2i-1} \},\qquad V_2:=\SPAN\{e_{2i-1}-i^{-1}e_{2i-1} \}.
\]
Then \(V=V_1+V_2\) is a dense subspace of \(\ell^2\) and the inverse \(S^{-1}\) is unbounded.

\change{}{Note that in the SSC method it is possible to make things go badly by choosing 
\(v\) and the spaces \(V_1,\dots,V_n\) so that the error reduction for \(v\)
goes to \(0\) as \(n\) goes to infinity.
The counterexample in \(\R^2\) can be made by choosing as the \(V_i\) uniformly
distributed rays. If the first space is almost orthogonal to \(v\) and the corrections
are done counterclockwise on the rays then as \(n\) goes to infinity
the subspace corrections are almost orthogonal to \(v\) and make it rotate.
}


As a last part of the geometrical interpretation we characterize the
minimal norm of a right-inverse of \(S\).

\begin{prop}
    The minimal norm for the right-inverses of \(S\) is
    \[
    \min\{\n{G}_{V\to \wV}: SG=\Id\} = \C_{\min}^{-1} 
    \]
    where
    \[
    \C_{\min}:= \inf_{v\ne 0 \in V}\max_i \sup_{w_i\ne 0\in V_i} \frac{(v,w_i)_V}{\n{w_i}_V \n{v}_V}.
    \]
\end{prop}
Note that \(0<\C_{\min}\le 1\) because \(V=\sum_iV_i\) and it is a 
measures of ``how well'' the collection of the \(V_i\) spans \(V\).
In the best case of a collection of orthogonal subspace then
clearly \(\C_{\min}=n^{-1/2}\).

\begin{proof}
    For \(\theta\in [0,\pi/2]\) let \(Y_\theta v\) be the set of vectors
    with angle less then \(\theta\) from \(\SPAN \{v\}\)
    \[Y_\theta v= \{w\in V:    (v,w)\ge \cos(\theta)\n{v}_V\n{w}_V \}.\]
    Let also \(\bar\theta=\cos^{-1} \C_{\min}\). By definition we have 
    \[
        \C_{\min}=\cos(\min\{\theta: \bigcup_i Y_\theta V_i= V\}) =\cos \bar\theta.
    \]
    so that
    \[
        V_{\min}= \bigcap_{\theta<\bar\theta} (V\setminus    \bigcup_i Y_\theta V_i) 
    \]
    is a union of lines through the origin.

    Fix \(f\in V_{\min}\) then the tangent hyper-plane to \(V_{\min}\) at
    \(f\) is the intersection  of the tangents of the \(\partial Y_{\bar\theta} V_i \}\)
     and consequently \(H:= f+ \SPAN\{\gamma_j,\, j\in  J\}\) is the orthogonal to \(V_{\min}\)
    at \(f\).

    Blowing-up around \(f\) in \(H\) the \( Y_{\bar\theta} V_j\), \(j\in J\)
    are \(\# J\) half-spaces that cover \(H\) because \( H \cap V_{\min}=\{f\} \).
    Since \(m\) half-spaces cannot cover \(\R^m\), \(\dim H<\# J\) and there exists
    a linear relation
    \[
    0=\sum_{j\in J}\alpha_j \gamma_j.    
    \]
    Let \(f_j\) be the orthogonal projection of \(f\) onto \(V_j\),
    by trigonometric considerations \(f+\tan(\bar\theta)\gamma_j = \cos(\bar\theta)^{-1} f_j \).
    Giving
    \[ \sum_{j\in J}  \alpha_j   f_j= c f.\] 
    Since the angle between \(f\) and \(f_j\) is \(\bar\theta\) all the 
    \(f_j\) have the same norm, namely \(\C_{\min} \n{f}_V\) and since their component
    on \(f\) is thus  \(\C_{\min}^2 \n{f}_V\) we have
    \[
        f=    c^-1 \sum_{j\in J}  \alpha_j   f_j,\qquad c=\C_{\min}^{-2} (\sum \alpha_j)^{-1}
    \]
    It follows that the claim is satisfied for \(f \in V_{\min}\) and \(\wv\in S^{-1}f\)
    defined as
    \[ w_i=\alpha_i \C_{\min}^{-2} (\sum \alpha_i)^{-1}.
    \]

    DA DIMOSTRARE PER QUELLI NON IN \(V_{\min}\).

\end{proof}



\subsection{Geometric interpretation}
\marginpar{QUESTA SEZ DOVREBBE SOSTITUIRE COROLLARY 2...}
Lemma~\ref{thm:stable-decomposition} allow the characterization of the
the extrema of the \(\spectrum(\Tp)\) for operators that can be diagonalized.
Recalling Lemma~\ref{thm:stable-decomposition} we have 
\((T^{-1}v,v)_V=\inf_{\wv\in S^{-1} v} \sum_{i=1}^n(T_i^{-1} v_i,v_i)_V\)
Consequently for any right-inverse, not necessarily linear, \(G\) of \(S\) we
get an upper bound of the form 
\[ (\Tp^{-1} v,v)_V \le  \sum_i (T_i^{-1} (G v)_i, (G v)_i)_V. \]
This leads to the following result.

\begin{prop}\label{thm:psc-lower-estimate}
    For any right-inverse \(G\) of \(S\) it holds
\[
    (\min \spectrum(\Tp))^{-1} \le \n{G}_{V\to\wV}^2 \max\{\n{T_i^{-1}}_{V_i\to V_i}, i=1,\dots,n \}.
\]
\end{prop}
\begin{proof}
Let \(\wv= G v\), then
\[\begin{aligned}
    (T^{-1}v,v)_V \le&  \sum_{i=1}^n(T_i^{-1} v_i,v_i)_V\le \max\{\n{T_i^{-1}}_{V_i\to V_i}, i=1,\dots,n \} \sum_i \n{v_i}^2
    \\&\le \max\{\n{T_i^{-1}}_{V_i\to V_i}, i=1,\dots,n \}(\sum_i \n{v_i}_V)^2 
    \\&\le \max\{\n{T_i^{-1}}_{V_i\to V_i}, i=1,\dots,n \} \n{G}_{V\to\wV}^2 \n{v}_V^2.
\end{aligned}
\]
\end{proof}

Introducing the cosine between the spaces \(V_i\) and \(V_j\)  
\[
\C_{i,j}:=\sup_{\substack{u_i\in V_i\\v_j\in V_j}} \frac{a(u_i,v_j)}{\n{u_i}_a \n{v_j}_a}\le 1
\]
one can achieve an upper bound for \(\spectrum(\Tp)\).
Note that the matrix \(\C\) is the identity if and only if the \(V_i\)
are mutually orthogonal. \change{}{and in general  \(\C\)  is a measure of  the redundancy
of the generating set \(\wPhi\).}

\begin{prop}\label{thm:psc-upper-estimate}
    For any right-inverse \(G\) of \(S\) it holds
\[
    (\max \spectrum(\Tp)) \le \n{G}_{V\to\wV}  \max\{\n{T_i}_{V\to V_i}, i=1,\dots,n \} \max_j\{\sum_i \C_{i,j}\} .
\]
\end{prop}
\begin{proof}
Let \(v\in V\) have norm 1 and \(\wv= G v\), then
\[\begin{aligned}
    (T v,v)_V &= \sum_{i,j}(T_i v, v_j)_V \le \max\{\n{T_i }_{V \to V_i}, i=1,\dots,n \} \sum_{i,j} \C_{i,j} \n{v_j}_V
    \\&\le\n{G}_{V\to\wV}  \max\{\n{T_i}_{V\to V_i}, i=1,\dots,n \} \max_j\{\sum_i \C_{i,j}\}.
\end{aligned}
\]
\end{proof}

The previous Propositions relate the spectrum of \(\Tp\) with the norm
the minimal norm of a right-inverse of \(S\), and in the following this 
is bounded with trigonometric terms.

\begin{prop}
    The minimal norm for the right-inverses of \(S\) is bounded
    \[
    \min\{\n{G}_{V\to \wV}: SG=\Id\} \le \frac2{\C_{\min}}
    \]
    where
    \[
    \C_{\min}:= \inf_{v\ne 0 \in V}\max_i \sup_{w_i\ne 0\in V_i} \frac{(v,w_i)_V}{\n{w_i}_V \n{v}_V}.
    \]
\end{prop}
Note that \(0<\C_{\min}\le 1\) because \(V=\sum_iV_i\) and it is a 
measures of ``how well'' the collection of the \(V_i\) spans \(V\).
In the best case of a collection of orthogonal subspace then
clearly \(\C_{\min}=n^{-1/2}\).\marginpar{NON SCALABILE ? Perche nella
prec. analisi (``old removed'') non compare $\n{G}_{V\to \wV}^3$? ma
se gli spazi sono ortogonali e usiamo la norma hilbertiana deve essere
$\n{G}_{V\to \wV}=1$ non $\n{G}_{V\to \wV}\simeq n^{-1/2}$  !? }

\begin{proof}
    It is sufficient to apply the \emph{greedy-SSC} method \cite{greedy-ssc},
    as a non-linear inverse of \(S\). 
    This corresponds to the problem~\ref{eq:system-wV} for \(A\) the adjoint of
    the Riesz isomorphism \(V^*\to V\) and \(T_i\) is the orthogonal projection
    on \(V_i\).
    It is well known that the method converges to a solution \(\wv\in S^{-1}v\).

    In the greedy-SSC the sequence of correction is adapted to the residual
    and maximizes the norm of the correction at each step.
    Let \(\wv^{[s]}\in \wV\) be the sequence of solutions generated by the method
    that is 
    \[
        \wv^{[s]}=\wv^{[s-1]}+\wT_{i_s}  (S^{*}v- \wT\wv^{[s]}),
    \]
    where \(i_s\) maximizes \(\n{S \wT_{i_s} (S^{*}v- \wT\wv^{[s]})}_V\).
   

    By assumption \(\n{S \wT_{i_s} (S^{*}v- \wT\wv^{[s]})}_V \ge \C_{\min} \n{(S^{*}v- \wT\wv^{[s]})}_V\)
    and by Pythagoras' theorem
    \[
        \n{S \wT_{i_s} (S^{*}v- \wT\wv^{[s]})}_V\le (1-\C_{\min}^2)^{1/2}    \n{(S^{*}v- \wT\wv^{[s]})}_V.
    \]
    The conclusion follows from triangular inequality 
    \[\begin{aligned}
        \n{\wv}_{\wV}&\le \sum_{s=0}^\infty \n{\wT_{i_s} (S^{*}v- \wT\wv^{[s]})}_{\wV}
         \le \C_{\min} \sum_{s=0}^\infty (1-\C_{\min}^2)^{i/2} \n{v}_V 
         \\&\le \frac{\C_{\min}}{1-(1-\C_{\min}^2)^{1/2}} = \frac{1+(1-\C_{\min}^2)^{1/2}}{\C_{\min}}.
    \end{aligned}\]
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "easy_adaptivity_and_solver_v6"
%%% End:


==> subspace-methods.tex <==
% !TEX root = easy_adaptivity_and_solver_v7.tex

\section{Subspace correction methods}

Subspace correction methods\cite{ssc-apm} are a family of operators built 
from a chosen preconditioners \(B_i:V_i^*\rightarrow V_i\) for the restriction of \(A\)
to the subspaces \(V_i\).
The aim of this section is to recall and rephrase them in the current framework, with the
aim of highlighting the effect of the geometry of the spaces \(V_i\) and of the
local preconditioners \(B_i\). 
The main subspace correction methods are the \emph{parallel subspace correction} (PSC),
and the many variations of the  \emph{successive subspace correction} (SSC).
Both methods fit very well in the proposed framework.

% \begin{remark}
% In the following the preconditioners and opertators adopting these methods will be
% labeled with ``PSC'' and ``SSC'' subscripts. 
% \end{remark}

For each \(B_i\) we define the corresponding  block diagonal operator in the extended space
\begin{equation}[wBi]
\wB_i:=\begin{pmatrix}
0 & \dots & 0\\ 
 \vdots &B_i & \vdots\\
  0 & \dots &0 
  \end{pmatrix}.
\end{equation}
and the following operators 
\[
     T_i:=  S \wB_i S^*A,\quad\text{and}\quad\wT_i:=\wB_i\wA.
\]

The PSC preconditioner is 
\begin{equation}[wB-PSC]
\wBp:=\begin{pmatrix}
B_1 & 0 & \dots & 0\\ 
 0 &\ddots & \ddots &\vdots\\
 \vdots & \ddots&\ddots &0\\
  0 & \dots &0 & B_n
  \end{pmatrix}=\sum_{i=1}^n \wB_i,
\end{equation} 
and it is also known as additive Schwarz preconditioner or as inexact
block-Jacobi solver. The preconditoned operator is
\begin{displaymath}
  \wTp := \wBp  \wA =\sum_{i=1}^n \wT_i.
\end{displaymath}


The SSC preconditioner $\wBs  $, also known as multiplicative Schwarz
preconditioner or inexact block-Gauss-Seidel solver,  gives  \(\ww=\wBs \wv\) as 
\begin{center}
  \begin{algorithmic}[c]
	\State $\ww\gets 0$
	\For {$j=1,\dots,r$}
	\State $\wt\gets \wB_{i_j} \wv$
 	\State $\ww\gets \ww + \wt$
	\State $\wv\gets \wv- \wA \wt$
\EndFor
\end{algorithmic}
\end{center}
where \((i_1,\dots,i_r)\) defines the sequence of subspace
corrections. In closed form it is then
\begin{equation}[wB-SSC]
\wBs:=\sum_{j=1}^r \wB_{i_j} \prod_{\ell=1}^{j-1}(\wId-\wA \wB_{i_\ell}).
\end{equation}
The preconditoned operator now reads 
\begin{displaymath}
  \wTs: = \wBs  \wA  = \sum_{j=1}^r \wT_{i_j}
  \prod_{\ell=1}^{j-1}(\wId-\wT_{i_\ell}) ,
\end{displaymath}  and the corresponding error operator  \(\wEs \) shows the link to an alternating projection method for the
error:
\[
  \wEs :=\wId - \wTs =\prod_{j=1}^r (\wId - \wT_{i_j}) .
\]

\color{blue}\marginpar{Fix symmetric SSC}
The \emph{forward} SSC corresponds to \(r=n\) and \(i_j=j\), the \emph{backward}
to \(r=n\) and \(i_j=n+1-j\).
To obtain the \emph{symmetric} SSC preconditioner one applies the forward SSC, multiplies the result by the diagonal blocks of $\wA$ and applies the backward SSC.
%The usual choice  corresponds to \(r=n\) and \(i_j=j\), while  the \emph{symmetric} SSC corresponds
%to \(r=2n-1\), \(i_j=j,\, j=1,\dots,n\), and \(i_j=2n-j,\,
%j=n+1,\dots,2n-1\), and 
Nonlinear variants exists, where the sequence of subspace corrections
is adapted to the right hand side,  e.g. with the 
\emph{greedy}-SSC \cite{greedy-ssc} where $r$ is determined by a tolerance and
\[
i_{j+1}:=\argmin\{\n{{\wEs}_{(i_1,\dots,i_{j},s)}\wy}_{\wV^*}: s=1,\dots,n\}.
\]
\color{black}

\subsection{Elliptic self-adjoint problems}

If \(A\) is a self-adjoint and coercive operator on \(V\) then it defines a norm \(\n{\cdot}_A\).
As common the analysis can thus be done in the \(A\)-induced norm and in this sub-section
it is assumed that \(A\) is the Riesz isomorphism for \(V^*\),
i.e. that \(\n{\cdot}_V=\n{\cdot}_A\).

The spectrum of \(\Tp\) and the norm of \(\Es\) are usually analyzed in terms 
that involve the geometry of the subspaces \(V_i\), the operator \(A\), and the
local preconditioners \(B_i\).
Three common references are \cite{Xu1992}, \cite{ssc-apm} and \cite{MR2104179}
where the assumptions vary slightly according to the different focus.
Here we take a even slightly different apprach that highlights separately the
effects of the choice of the  \(V_i\)  and of the quality of the local
preconditioners \(B_i\). 
For completeness the implication from the presented formulation to the ``standard''
assumptions is included.

\begin{thm}\label{thm:classical-result}
If \(A\), and the \(B_i\) are self-adjoint and coercive then 
\begin{align}
\label{eq:Tp-lower}& \min \spectrum(\Tp)\ge \lambda_{\min}  K^{-2},\\
\label{eq:Tp-upper}& \max \spectrum(\Tp)\le \lambda_{\max} \n{\C}_{\R^n\to\R^n},\\
\label{eq:Es-upper}& \n{\Es}_{V\to V}\le 1-\frac{\lambda_{\min}(2-\lambda_{\max})}{K^2 (1+\lambda_{\max} \n{\C}_{\R^n\to\R^n})^2},
\end{align}
where \(K, \lambda_{\min},\lambda_{\max} \in \R\) and \(\C\in\R^{n\times n}\) 
are respectively 
\begin{itemize}
\item the \emph{stable-decompositions} constant
\begin{equation}\label{eq:stable-dec} 
K:=\inf_{SG=\Id}\n{G}_{V\to\wV},
%\exists \sum_{i=1}^n (B_i^{-1} v_i,v_i)_V  \le K_0 (A v,v)_V,
\end{equation}
\item the \emph{local stability} constants
\begin{align}
\label{eq:lmin} \lambda_{\min}&:=\min\{\n{T_i^{-1}}_{V_i\to V_i}^{-1},\,i=1,\dots,n\},\\ 
\label{eq:lmax} \lambda_{\max}&:=\max\{\n{T_i}_{V_i\to V_i},\,i=1,\dots,n\}.
\end{align}
\item the \emph{strengthned Cauchy-Schwarz-inequality} symmetric matrix
\begin{equation}
\label{eq:s-cauchy-schwarz}
\C_{i,j}:=\sup_{\substack{u_i\in V_i\\v_j\in V_j}} \frac{(u_i,v_j)_V}{\n{u_i}_V \n{v_j}_V}\in [0, 1].
%\sum_{i=1}^n\sum_{j=1}^n (T_i v_i,T_j w_j)_A \le K_1 \Big(\sum_{i=1}^n (T_i v_i,v_i)_A\Big )^{1/2}\Big(\sum_{i=1}^n (T_i w_i,w_i)_A\Big )^{1/2},
\end{equation}
\end{itemize}
\end{thm}

\begin{remark} The strengthned Cauchy-Schwarz-inequality and stable-decompositions
emphasise  the role of the  \(V_i\), while the local stability emphasise the
quality of the preconditioners \(B_i\).
\end{remark}



The above results and Theorems~\ref{thm:krylov-iteration-CG}--\ref{thm:preconditioner-spectrum}
lead to the following estimates for \(\wTp\) and \(\wTs\).
\begin{cor}\label{thm:PSC-summary}
The conditioning of the PSC method is bounded by
\begin{equation}
  \label{eq:PSC-bound}
  \frac{\max \spectrum(\wTp)}{\min \spectrum(\wTp)\setminus\{0\}}\le\underbrace{K^2 \n{\C}_{\R^n\to \R^n}}_{\text{geometry of the }V_i}\underbrace{\lambda_{\max}\lambda_{\min}^{-1}}_{\text{quality of the } B_i}
\end{equation}
and the error operator
of the SSC method is bounded by
\begin{displaymath}
  \n{S\wEs^k}_{\wV\to V}\le \n{\Es}_{V\to V}^k.
\end{displaymath}

\end{cor}

The proof of \eqref{eq:Tp-lower} follows from the technical lemma and
corollary below
\begin{lem}[{\cite[Lemma~2.4]{ssc-apm}}]\label{thm:stable-decomposition}
If \(\Tp\) is an isomorphism and each \(T_i\) is self-adjoint and coercive \(V_i \to V_i\), then
    \[
        (\Tp^{-1}v,v)_V=\inf_{\wv\in S^{-1} v} \sum_{i=1}^n(T_i^{-1} v_i,v_i)_V= \sum_{i=1}^n (T_i^{-1} w_i,w_i)_V,
    \]
where \(w_i=T_i\Tp^{-1}v\).
\end{lem}

\begin{cor}\label{thm:psc-lower-estimate}
For any right-inverse \(G\) of \(S\) it holds
\[
    (\min \spectrum(\Tp))^{-1}\le  \lambda_{\min}\n{G}_{V\to\wV}^2.
\]
\end{cor}
\begin{proof}
Let \(\n{v}_V=1\) and \(\wv=(v_1,\dots,v_n)= G v\), then
\[\begin{aligned}
    (\Tp^{-1}v,v)_V \le&  \sum_{i=1}^n(T_i^{-1} v_i,v_i)_V\le \max\{\n{T_i^{-1}}_{V_i\to V_i}, i=1,\dots,n \} \sum_i \n{v_i}^2
    \\&\le  \lambda_{\min}^{-1} \n{\wv}_{\wV}^2  \le \lambda_{\min}^{-1} \n{G}_{V\to\wV}^2.
\end{aligned}
\]
\end{proof}

To prove \eqref{eq:Tp-upper} and \eqref{eq:Es-upper} we recall
\cite[Equation~(2.15)]{MR2104179} where \(P_i\) corresponds to \(T_i\)
and \(\omega\) to \(\lambda_{\max}\) so that it reads: \(\forall i=1,\dots,n,\,\forall v\in V\)
\[
(T_i v,T_i v)_V^{1/2}\le \lambda_{\max}(T_i v,v)_V^{1/2}.
\]
Then we have 
\begin{equation}
(T_i v, T_j w)_V\le \C_{i,j} (T_i v,T_i v)_V^{1/2} (T_j w,T_j w)_V ^{1/2} \le \lambda_{\max}\C_{i,j} (T_i v,v)_V^{1/2} (T_j w,w)_V ^{1/2}
\end{equation}
that is \cite[Equation~(4.10)]{Xu1992} with \(\omega=\lambda_{\max}\) and \(\epsilon_{i,j}=\C_{i,j}\).
Consequently \cite[Lemma~4.6, Thorem~4.1 and Theorem~4.6]{Xu1992} apply with
\(K_1=\lambda_{\max}\n{\C}_{\R^n\to\R^n}\) and \(K_0=\lambda_{\min}^{-1}K^2\).




